Systematic Broad-band X-ray Study of super-Eddington Accretion onto Supermassive Black Holes. I. X-ray Continuum

We present the first systematic broad-band X-ray study of super-Eddington accretion onto SMBHs with simultaneous {\it NuSTAR} and {\it XMM-Newton} or {\it Swift}/XRT observations of a sample of 8 super-Eddington accreting AGN with Eddington ratio $1<\lambda_{\rm Edd}<426$. We find that the SEAMBHs show a steep primary continuum slope as expected for sources accreting in the super Eddington regime, mostly dominated by relativistic reflection. The Iron K$\alpha$ emission lines of the sources of our sample show relativistic broadening. In addition the equivalent widths of the narrow components of the Iron K$\alpha$ lines follow the 'X-ray Baldwin' effect, also known as the 'Iwasawa-Taniguchi' effect. We found a statistically significant correlation between the photon-index of the primary power-law and the Eddington ratio, consistent with past studies. Moreover, as expected for super-Eddington sources, the median value of the reflection fraction of the sources we analysed is a factor $\sim 2$ higher than the median reflection fraction value of the type\,1 AGN from the BASS sample. We are able to estimate the coronal temperature for three sources of our sample: Mrk\,382 ($kT_e=7.8$\,keV), PG\,0026+129 ($kT_e=39$\,keV) and IRAS\,04416+1215 ($kT_e=3$\,keV). Looking at the position of the SEAMBHs sources of our sample in the compactness-temperature diagram it appears that in super-Eddington AGN, as for lower Eddington ratio AGN, the X-ray corona is controlled by pair production and annihilation.

==> bibliography.tex <==
@INPROCEEDINGS{Gabriel2004,
       author = {{Gabriel}, C. and {Denby}, M. and {Fyfe}, D.~J. and {Hoar}, J. and {Ibarra}, A. and {Ojero}, E. and {Osborne}, J. and {Saxton}, R.~D. and {Lammers}, U. and {Vacanti}, G.},
        title = "{The XMM-Newton SAS - Distributed Development and Maintenance of a Large Science Analysis System: A Critical Analysis}",
    booktitle = {Astronomical Data Analysis Software and Systems (ADASS) XIII},
         year = 2004,
       editor = {{Ochsenbein}, Francois and {Allen}, Mark G. and {Egret}, Daniel},
       series = {Astronomical Society of the Pacific Conference Series},
       volume = {314},
        month = jul,
        pages = {759},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004ASPC..314..759G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Piconcelli2004,
       author = {{Piconcelli}, E. and {Jimenez-Bail{\'o}n}, E. and {Guainazzi}, M. and {Schartel}, N. and {Rodr{\'\i}guez-Pascual}, P.~M. and {Santos-Lle{\'o}}, M.},
        title = "{Evidence for a multizone warm absorber in the XMM-Newton spectrum of Markarian 304}",
      journal = {\mnras},
     keywords = {galaxies: active, galaxies: individual: Markarian 304, galaxies: Seyfert, X-rays: galaxies, Astrophysics},
         year = 2004,
        month = jun,
       volume = {351},
       number = {1},
        pages = {161-168},
          doi = {10.1111/j.1365-2966.2004.07764.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0404263},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004MNRAS.351..161P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{1972ApJ...171..467B,
       author = {{Bahcall}, John N. and {Kozlovsky}, Ben-Zion and {Salpeter}, E.~E.},
        title = "{On the Time Dependence of Emission-Line Strengths from a Photoionized Nebula}",
      journal = {\apj},
         year = 1972,
        month = feb,
       volume = {171},
        pages = {467},
          doi = {10.1086/151300},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1972ApJ...171..467B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2019ApJ...870L..13A,
       author = {{Adegoke}, Oluwashina and {Dewangan}, Gulab C. and {Pawar}, Pramod and {Pal}, Main},
        title = "{UV to X-Ray Comptonization Delay in Mrk 493}",
      journal = {\apjl},
     keywords = {galaxies: active, galaxies: individual: Mrk 493, galaxies: Seyfert, X-rays: galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2019,
        month = jan,
       volume = {870},
       number = {2},
          eid = {L13},
        pages = {L13},
          doi = {10.3847/2041-8213/aaf8ab},
archivePrefix = {arXiv},
       eprint = {1812.08056},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...870L..13A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2020Univ....6..136F,
       author = {{Foschini}, Luigi},
        title = "{Jetted Narrow-Line Seyfert 1 Galaxies \& Co.: Where Do We Stand?}",
      journal = {Universe},
     keywords = {Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Astrophysics of Galaxies},
         year = 2020,
        month = aug,
       volume = {6},
       number = {9},
        pages = {136},
          doi = {10.3390/universe6090136},
archivePrefix = {arXiv},
       eprint = {2008.13383},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020Univ....6..136F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{1999ApJ...521L..95P,
       author = {{Peterson}, Bradley M. and {Wandel}, Amri},
        title = "{Keplerian Motion of Broad-Line Region Gas as Evidence for Supermassive Black Holes in Active Galactic Nuclei}",
      journal = {\apjl},
     keywords = {GALAXIES: ACTIVE, GALAXIES: INDIVIDUAL: NGC NUMBER: NGC 5548, GALAXIES: SEYFERT, GALAXIES: QUASARS: EMISSION LINES, Galaxies: Active, Galaxies: Individual: NGC Number: NGC 5548, Galaxies: Seyfert, Galaxies: Quasars: Emission Lines, Astrophysics},
         year = 1999,
        month = aug,
       volume = {521},
       number = {2},
        pages = {L95-L98},
          doi = {10.1086/312190},
archivePrefix = {arXiv},
       eprint = {astro-ph/9905382},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1999ApJ...521L..95P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1985ApJ...297..166O,
       author = {{Osterbrock}, D.~E. and {Pogge}, R.~W.},
        title = "{The spectra of narrow-line Seyfert 1 galaxies.}",
      journal = {\apj},
     keywords = {Astronomical Spectroscopy, Galactic Nuclei, Seyfert Galaxies, Abundance, Active Galactic Nuclei, Emission Spectra, H Beta Line, Hydrogen Ions, Iron, Luminosity, Spectral Energy Distribution, Spectral Line Width, Astrophysics},
         year = 1985,
        month = oct,
       volume = {297},
        pages = {166-176},
          doi = {10.1086/163513},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1985ApJ...297..166O},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{10.1093/mnras/sty971,
    author = {Wu, Samantha and Coughlin, Eric R and Nixon, Chris},
    title = "{Super-Eddington accretion in tidal disruption events: the impactof realistic fallback rates on accretion rates}",
    journal = {Monthly Notices of the Royal Astronomical Society},
    volume = {478},
    number = {3},
    pages = {3016-3024},
    year = {2018},
    month = {04},
    abstract = "{After the tidal disruption of a star by a massive black hole, disrupted stellar debris can fall back to the hole at a rate significantly exceeding its Eddington limit. To understand how black hole mass affects the duration of super-Eddington accretion in tidal disruption events, we first run a suite of simulations of the disruption of a Solar-like star by a supermassive black hole of varying mass to directly measure the fallback rate on to the hole, and we compare these fallback rates to the analytic predictions of the ‘frozen-in’ model. Then, adopting a zero-Bernoulli accretion flow as an analytic prescription for the accretion flow around the hole, we investigate how the accretion rate on to the black hole evolves with the more accurate fallback rates calculated from the simulations. We find that numerically simulated fallback rates yield accretion rates on to the hole that can, depending on the black hole mass, be nearly an order of magnitude larger than those predicted by the frozen-in approximation. Our results place new limits on the maximum black hole mass for which super-Eddington accretion occurs in tidal disruption events.}",
    issn = {0035-8711},
    doi = {10.1093/mnras/sty971},
    url = {https://doi.org/10.1093/mnras/sty971},
    eprint = {https://academic.oup.com/mnras/article-pdf/478/3/3016/25063038/sty971.pdf},
}
@article{begelman2006,
    author = {Begelman, M. C. and King, A. R. and Pringle, J. E.},
    title = "{The nature of SS433 and the ultraluminous X-ray sources}",
    journal = {Monthly Notices of the Royal Astronomical Society},
    volume = {370},
    number = {1},
    pages = {399-404},
    year = {2006},
    month = {07},
    abstract = "{The periodic precession (162-d) and nodding (6.3-d) motions of the jets in SS433 are driven in the outer regions of the disc, whereas the jets themselves, being relativistic, are launched near the black hole at the disc centre. Given that the nutation period is comparable to the dynamical time-scale in the outer regions of the disc, it seems unlikely that these periods can be communicated efficiently to the disc centre. Here, we propose that the massive outflow observed in SS433 is launched at large radii in the disc, about 1/10 of the outer disc edge, and that it is this outflow which responds to the oscillations of the outer disc and determines the direction of the jets. The massive outflow is launched at large radius because the mass transfer rate is hyper-Eddington. This implies not only that the total luminosity of SS433 exceeds LEdd by a considerable factor, but also that the radiative output is collimated along the outflow. We thus suggest that SS433 is an ultraluminous X-ray source (ULX) viewed ‘from the side’. We also suggest that the obscured INTEGRAL sources may be SS433-like objects, but with slightly lower mass transfer rates.}",
    issn = {0035-8711},
    doi = {10.1111/j.1365-2966.2006.10469.x},
    url = {https://doi.org/10.1111/j.1365-2966.2006.10469.x},
    eprint = {https://academic.oup.com/mnras/article-pdf/370/1/399/3415273/mnras0370-0399.pdf},
}
@article{Assef_2015,
	doi = {10.1088/0004-637x/804/1/27},
	url = {https://doi.org/10.1088/0004-637x/804/1/27},
	year = 2015,
	month = {apr},
	publisher = {American Astronomical Society},
	volume = {804},
	number = {1},
	pages = {27},
	author = {R. J. Assef and P. R. M. Eisenhardt and D. Stern and C.-W. Tsai and J. Wu and D. Wylezalek and A. W. Blain and C. R. Bridge and E. Donoso and A. Gonzales and R. L. Griffith and T. H. Jarrett},
	title = {{HALF} {OF} {THE} {MOST} {LUMINOUS} {QUASARS} {MAY} {BE} {OBSCURED}: {INVESTIGATING} {THE} {NATURE} {OFWISE}-{SELECTED} {HOT} {DUST}-{OBSCURED} {GALAXIES}},
	journal = {The Astrophysical Journal},
	abstract = {The Wide-field Infrared Survey Explorer mission has unveiled a rare population of high-redshift (z = 1–4.6), dusty, hyper-luminous galaxies, with infrared luminosities , and sometimes exceeding . Previous work has shown that their dust temperatures and overall far-infrared spectral energy distributions (SEDs) are significantly hotter than expected to be powered by star formation. We present here an analysis of the rest-frame optical through mid-infrared SEDs for a large sample of these so-called “hot, dust-obscured galaxies” (Hot DOGs). We find that the SEDs of Hot DOGs are generally well modeled by the combination of a luminous, yet obscured active galactic nuclei (AGNs) that dominates the rest-frame emission at and the bolometric luminosity output, and a less luminous host galaxy that is responsible for the bulk of the rest optical/UV emission. Even though the stellar mass of the host galaxies may be as large as 1011–1012 M⊙, the AGN emission, with a range of luminosities comparable to those of the most luminous QSOs known, require that either Hot DOGs have black hole masses significantly in excess of the local relations, or that they radiate significantly above the Eddington limit, at a level at least 10 times more efficiently than z ∼ 2 QSOs. We show that, while rare, the number density of Hot DOGs is comparable to that of equally luminous but unobscured (i.e., Type 1) QSOs. This may be at odds with the trend suggested at lower luminosities for the fraction of obscured AGNs to decrease with increasing luminosity. That trend may, instead, reverse at higher luminosities. Alternatively, Hot DOGs may not be the torus-obscured counterparts of the known optically selected, largely unobscured, hyper-luminous QSOs, and may represent a new component of the galaxy evolution paradigm. Finally, we discuss the environments of Hot DOGs and statistically show that these objects are in regions as dense as those of known high-redshift proto-clusters.}
}
@ARTICLE{2012Sci...337..544V,
       author = {{Volonteri}, M.},
        title = "{The Formation and Evolution of Massive Black Holes}",
      journal = {Science},
     keywords = {ASTRONOMY, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2012,
        month = aug,
       volume = {337},
       number = {6094},
        pages = {544},
          doi = {10.1126/science.1220843},
archivePrefix = {arXiv},
       eprint = {1208.1106},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012Sci...337..544V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2017ApJ...850...74K,
       author = {{Koss}, Michael and {Trakhtenbrot}, Benny and {Ricci}, Claudio and {Lamperti}, Isabella and {Oh}, Kyuseok and {Berney}, Simon and {Schawinski}, Kevin and {Balokovi{\'c}}, Mislav and {Baronchelli}, Linda and {Crenshaw}, D. Michael and {Fischer}, Travis and {Gehrels}, Neil and {Harrison}, Fiona and {Hashimoto}, Yasuhiro and {Hogg}, Drew and {Ichikawa}, Kohei and {Masetti}, Nicola and {Mushotzky}, Richard and {Sartori}, Lia and {Stern}, Daniel and {Treister}, Ezequiel and {Ueda}, Yoshihiro and {Veilleux}, Sylvain and {Winter}, Lisa},
        title = "{BAT AGN Spectroscopic Survey. I. Spectral Measurements, Derived Quantities, and AGN Demographics}",
      journal = {\apj},
     keywords = {black hole physics, galaxies: active, galaxies: nuclei, quasars: general, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Astrophysics of Galaxies},
         year = 2017,
        month = nov,
       volume = {850},
       number = {1},
          eid = {74},
        pages = {74},
          doi = {10.3847/1538-4357/aa8ec9},
archivePrefix = {arXiv},
       eprint = {1707.08123},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...850...74K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2013ARA&A..51..511K,
       author = {{Kormendy}, John and {Ho}, Luis C.},
        title = "{Coevolution (Or Not) of Supermassive Black Holes and Host Galaxies}",
      journal = {\araa},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2013,
        month = aug,
       volume = {51},
       number = {1},
        pages = {511-653},
          doi = {10.1146/annurev-astro-082708-101811},
archivePrefix = {arXiv},
       eprint = {1304.7762},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ARA&A..51..511K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{1998A&A...333..827G,
       author = {{Grupe}, D. and {Wills}, Beverley J. and {Wills}, D. and {Beuermann}, K.},
        title = "{Scattering and absorption in soft X-ray selected AGN: an optical polarization survey}",
      journal = {\aap},
     keywords = {POLARIZATION, GALAXIES: ACTIVE, GALAXIES: NUCLEI, GALAXIES: SEYFERT, Astrophysics},
         year = 1998,
        month = may,
       volume = {333},
        pages = {827-840},
archivePrefix = {arXiv},
       eprint = {astro-ph/9712149},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1998A&A...333..827G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{1992A&A...262...49S,
       author = {{Singh}, K.~P. and {Rao}, A.~R. and {Vahia}, M.~N.},
        title = "{EXOSAT measurement of the spectrum of Markarian 382.}",
      journal = {\aap},
     keywords = {Exosat Satellite, Markarian Galaxies, Satellite Observation, X Ray Spectra, Galactic Nuclei, Seyfert Galaxies, Astrophysics},
         year = 1992,
        month = aug,
       volume = {262},
        pages = {49-51},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1992A&A...262...49S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{1988ApJ...330..178T,
       author = {{Treves}, A. and {Bouchet}, P. and {Chiappetti}, L. and {Ciapi}, A. and {Falomo}, R. and {Maraschi}, L. and {Tanzi}, E.~G.},
        title = "{The X-Ray to Infrared Energy Distribution of the Quasar PG 0026+129}",
      journal = {\apj},
     keywords = {Energy Distribution, Infrared Sources (Astronomy), Optical Emission Spectroscopy, Quasars, Stellar Spectrophotometry, X Ray Sources, Active Galactic Nuclei, Energy Bands, Exosat Satellite, Heao 2, Astrophysics, QUASARS, SPECTROPHOTOMETRY, X-RAYS: SOURCES},
         year = 1988,
        month = jul,
       volume = {330},
        pages = {178},
          doi = {10.1086/166464},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1988ApJ...330..178T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@article{Vasylenko2018,
   title={The broad-band spectrum of the narrow-line Seyfert 1 NGC 4748: from UV to hard X-ray},
   volume={363},
   ISSN={1572-946X},
   url={http://dx.doi.org/10.1007/s10509-018-3447-2},
   DOI={10.1007/s10509-018-3447-2},
   number={11},
   journal={Astrophysics and Space Science},
   publisher={Springer Science and Business Media LLC},
   author={Vasylenko, A. A.},
   year={2018},
   month={Oct}
}
@ARTICLE{2011MNRAS.417.2426P,
       author = {{Panessa}, F. and {de Rosa}, A. and {Bassani}, L. and {Bazzano}, A. and {Bird}, A. and {Landi}, R. and {Malizia}, A. and {Miniutti}, G. and {Molina}, M. and {Ubertini}, P.},
        title = "{Narrow-line Seyfert 1 galaxies at hard X-rays}",
      journal = {\mnras},
     keywords = {galaxies: active, galaxies: Seyfert, X-rays: galaxies, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2011,
        month = nov,
       volume = {417},
       number = {4},
        pages = {2426-2439},
          doi = {10.1111/j.1365-2966.2011.19268.x},
archivePrefix = {arXiv},
       eprint = {1106.3023},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011MNRAS.417.2426P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2010MNRAS.403..945L,
       author = {{Landi}, R. and {Bassani}, L. and {Malizia}, A. and {Stephen}, J.~B. and {Bazzano}, A. and {Fiocchi}, M. and {Bird}, A.~J.},
        title = "{Swift/XRT observations of unidentified INTEGRAL/IBIS sources}",
      journal = {\mnras},
     keywords = {catalogues, surveys, gamma-rays: observations, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Solar and Stellar Astrophysics},
         year = 2010,
        month = apr,
       volume = {403},
       number = {2},
        pages = {945-959},
          doi = {10.1111/j.1365-2966.2010.16183.x},
archivePrefix = {arXiv},
       eprint = {0912.1519},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010MNRAS.403..945L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2001A&A...368..797P,
       author = {{Pfefferkorn}, F. and {Boller}, Th. and {Rafanelli}, P.},
        title = "{Soft X-ray properties of a spectroscopically selected sample of interacting and isolated Seyfert galaxies}",
      journal = {\aap},
     keywords = {CATALOGS, GALAXIES: ACTIVE, GALAXIES: INTERACTIONS, GALAXIES: SEYFERT, X-RAYS: GALAXIES, Astrophysics},
         year = 2001,
        month = mar,
       volume = {368},
        pages = {797-816},
          doi = {10.1051/0004-6361:20010055},
archivePrefix = {arXiv},
       eprint = {astro-ph/0101184},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001A&A...368..797P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2004A&A...422...85P,
       author = {{Porquet}, D. and {Reeves}, J.~N. and {O'Brien}, P. and {Brinkmann}, W.},
        title = "{XMM-Newton EPIC observations of 21 low-redshift PG quasars}",
      journal = {\aap},
     keywords = {galaxies: quasars: general, X-rays: general, galaxies: nuclei, radiation mechanisms : general, Astrophysics},
         year = 2004,
        month = jul,
       volume = {422},
        pages = {85-95},
          doi = {10.1051/0004-6361:20047108},
archivePrefix = {arXiv},
       eprint = {astro-ph/0404385},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004A&A...422...85P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2000ApJ...531...52G,
       author = {{George}, I.~M. and {Turner}, T.~J. and {Yaqoob}, T. and {Netzer}, H. and {Laor}, A. and {Mushotzky}, R.~F. and {Nandra}, K. and {Takahashi}, T.},
        title = "{X-Ray Observations of Optically Selected, Radio-quiet Quasars. I. The ASCA Results}",
      journal = {\apj},
     keywords = {GALAXIES: ACTIVE, GALAXIES: NUCLEI, GALAXIES: QUASARS: GENERAL, X-RAYS: GALAXIES, Astrophysics},
         year = 2000,
        month = mar,
       volume = {531},
       number = {1},
        pages = {52-80},
          doi = {10.1086/308461},
archivePrefix = {arXiv},
       eprint = {astro-ph/9910218},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000ApJ...531...52G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@article{Li_2018,
	doi = {10.3847/1538-4357/aaee6b},
	url = {https://doi.org/10.3847/1538-4357/aaee6b},
	year = 2018,
	month = {dec},
	publisher = {American Astronomical Society},
	volume = {869},
	number = {2},
	pages = {137},
	author = {Yan-Rong Li and Yu-Yang Songsheng and Jie Qiu and Chen Hu and Pu Du and Kai-Xing Lu and Ying-Ke Huang and Jin-Ming Bai and Wei-Hao Bian and Ye-Fei Yuan and Luis C. Ho and Jian-Min Wang},
	title = {Supermassive Black Holes with High Accretion Rates in Active Galactic Nuclei. {VIII}. Structure of the Broad-line Region and Mass of the Central Black Hole in Mrk 142},
	journal = {The Astrophysical Journal},
	abstract = {This is the eighth in a series of papers reporting on a large reverberation mapping (RM) campaign to measure black hole (BH) mass in active galactic nuclei with high accretion rates. We employ the recently developed dynamical modeling approach for broad-line regions (BLRs) based on the method of Pancoast et al. to analyze the RM data set of Mrk 142 observed in the first monitoring season. In this approach, continuum variations are reconstructed using a damped random walk process, and BLR structure is delineated using a flexible disk-like geometry, in which BLR clouds move around the central BH with Keplerian orbits or inflow/outflow motion. The approach also includes the possibilities of anisotropic emission from BLR clouds, nonlinear response of the line emission to the continuum, and different long-term trends in the continuum and emission-line variations. We implement the approach in a Bayesian framework that is apt for parallel computation and use a Markov chain Monte Carlo technique to recover the parameters and uncertainties for the modeling, including the mass of the central BH. We apply three BLR models with different prescriptions of BLR cloud distributions and find that the best model for fitting the data of Mrk 142 is a two-zone BLR model, consistent with the theoretical BLR model surrounding slim accretion disks. The best model yields a BH mass of , resulting in a virial factor of for the full width at half maximum of the Hβ line measured from the mean spectrum. The virial factors for the other measures of the Hβ line width are also presented.}
}
@article{10.1093/mnrasl/slw030,
    author = {Barth, Aaron J. and Bentz, Misty C.},
    title = "{No evidence for [O iii] variability in Mrk 142}",
    journal = {Monthly Notices of the Royal Astronomical Society: Letters},
    volume = {458},
    number = {1},
    pages = {L109-L113},
    year = {2016},
    month = {02},
    abstract = "{Using archival data from the 2008 Lick AGN Monitoring Project, Zhang \\&amp; Feng claimed to find evidence for flux variations in the narrow [O iii] emission of the Seyfert 1 galaxy Mrk 142 over a two-month time span. If correct, this would imply a surprisingly compact size for the narrow-line region. We show that the claimed [O iii] variations are merely the result of random errors in the overall flux calibration of the spectra. The data do not provide any support for the hypothesis that the [O iii] flux was variable during the 2008 monitoring period.}",
    issn = {1745-3925},
    doi = {10.1093/mnrasl/slw030},
    url = {https://doi.org/10.1093/mnrasl/slw030},
    eprint = {https://academic.oup.com/mnrasl/article-pdf/458/1/L109/8011310/slw030.pdf},
}
@ARTICLE{2016MNRAS.457L..64Z,
       author = {{Zhang}, Xue-Guang and {Feng}, Long-Long},
        title = "{Apparent [O III] variability in the narrow line Seyfert I Mrk142}",
      journal = {\mnras},
     keywords = {galaxies: active, galaxies: nuclei, quasars: emission lines, galaxies: Seyfert, Astrophysics - Astrophysics of Galaxies},
         year = 2016,
        month = mar,
       volume = {457},
       number = {1},
        pages = {L64-L68},
          doi = {10.1093/mnrasl/slv204},
archivePrefix = {arXiv},
       eprint = {1512.07673},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016MNRAS.457L..64Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2018MNRAS.477.3247B,
       author = {{Bonson}, K. and {Gallo}, L.~C. and {Wilkins}, D.~R. and {Fabian}, A.~C.},
        title = "{Variable blurred reflection in the narrow-line Seyfert 1 galaxy Mrk 493}",
      journal = {\mnras},
     keywords = {galaxies: active, galaxies: individual: Mrk 493, galaxies: nuclei, galaxies: Seyfert, X-rays: galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2018,
        month = jul,
       volume = {477},
       number = {3},
        pages = {3247-3256},
          doi = {10.1093/mnras/sty828},
archivePrefix = {arXiv},
       eprint = {1803.10305},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018MNRAS.477.3247B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@article{Petrucci2018,
  TITLE = {{Testing warm Comptonization models for the origin of the soft X-ray excess in AGNs}},
  AUTHOR = {Petrucci, Pierre-Olivier and Ursini, F. and De Rosa, A. and Bianchi, S. and Cappi, M. and Matt, G. and Dadina, M. and Malzac, J.},
  URL = {https://hal.archives-ouvertes.fr/hal-03014216},
  JOURNAL = {{Astronomy and Astrophysics - A\\&A}},
  PUBLISHER = {{EDP Sciences}},
  VOLUME = {611},
  PAGES = {A59},
  YEAR = {2018},
  MONTH = Mar,
  DOI = {10.1051/0004-6361/201731580},
  KEYWORDS = {galaxies: active ; galaxies: Seyfert ; X-rays: galaxies},
  PDF = {https://hal.archives-ouvertes.fr/hal-03014216/file/aa31580-17.pdf},
  HAL_ID = {hal-03014216},
  HAL_VERSION = {v1},
}
@ARTICLE{Ursini2020,
       author = {{Ursini}, F. and {Dov{\v{c}}iak}, M. and {Zhang}, W. and {Matt}, G. and {Petrucci}, P. -O. and {Done}, C.},
        title = "{Estimating the size of X-ray lamppost coronae in active galactic nuclei}",
      journal = {\aap},
     keywords = {black hole physics, galaxies: active, galaxies: Seyfert, X-rays: galaxies, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Astrophysics of Galaxies},
         year = 2020,
        month = dec,
       volume = {644},
          eid = {A132},
        pages = {A132},
          doi = {10.1051/0004-6361/202039158},
archivePrefix = {arXiv},
       eprint = {2010.07166},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020A&A...644A.132U},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@INPROCEEDINGS{2007AAS...211.4418W,
       author = {{Wills}, Beverley J. and {Grupe}, D. and {Leighly}, K.},
        title = "{IRAS F12397+3333: Optical Spectropolarimetry \& X-ray Ionized Absorbers}",
    booktitle = {American Astronomical Society Meeting Abstracts},
         year = 2007,
       series = {American Astronomical Society Meeting Abstracts},
       volume = {211},
        month = dec,
          eid = {44.18},
        pages = {44.18},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007AAS...211.4418W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{pexrav,
       author = {{Magdziarz}, Pawel and {Zdziarski}, Andrzej A.},
        title = "{Angle-dependent Compton reflection of X-rays and gamma-rays}",
      journal = {\mnras},
     keywords = {RADIATION MECHANISMS: NONTHERMAL, SCATTERING, GALAXIES: SEYFERT, X-RAYS: GENERAL, GAMMA-RAYS: THEORY},
         year = 1995,
        month = apr,
       volume = {273},
       number = {3},
        pages = {837-848},
          doi = {10.1093/mnras/273.3.837},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1995MNRAS.273..837M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Kaspi2000,
       author = {{Kaspi}, Shai and {Smith}, Paul S. and {Netzer}, Hagai and {Maoz}, Dan and {Jannuzi}, Buell T. and {Giveon}, Uriel},
        title = "{Reverberation Measurements for 17 Quasars and the Size-Mass-Luminosity Relations in Active Galactic Nuclei}",
      journal = {\apj},
     keywords = {GALAXIES: ACTIVE, GALAXIES: QUASARS: EMISSION LINES, GALAXIES: QUASARS: GENERAL, Astrophysics},
         year = 2000,
        month = apr,
       volume = {533},
       number = {2},
        pages = {631-649},
          doi = {10.1086/308704},
archivePrefix = {arXiv},
       eprint = {astro-ph/9911476},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000ApJ...533..631K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Bentz2009,
       author = {{Bentz}, Misty C. and {Walsh}, Jonelle L. and {Barth}, Aaron J. and {Baliber}, Nairn and {Bennert}, Vardha Nicola and {Canalizo}, Gabriela and {Filippenko}, Alexei V. and {Ganeshalingam}, Mohan and {Gates}, Elinor L. and {Greene}, Jenny E. and {Hidas}, Marton G. and {Hiner}, Kyle D. and {Lee}, Nicholas and {Li}, Weidong and {Malkan}, Matthew A. and {Minezaki}, Takeo and {Sakata}, Yu and {Serduke}, Frank J.~D. and {Silverman}, Jeffrey M. and {Steele}, Thea N. and {Stern}, Daniel and {Street}, Rachel A. and {Thornton}, Carol E. and {Treu}, Tommaso and {Wang}, Xiaofeng and {Woo}, Jong-Hak and {Yoshii}, Yuzuru},
        title = "{The Lick AGN Monitoring Project: Broad-line Region Radii and Black Hole Masses from Reverberation Mapping of H{\ensuremath{\beta}}}",
      journal = {\apj},
     keywords = {galaxies: active, galaxies: nuclei, galaxies: Seyfert, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2009,
        month = nov,
       volume = {705},
       number = {1},
        pages = {199-217},
          doi = {10.1088/0004-637X/705/1/199},
archivePrefix = {arXiv},
       eprint = {0908.0003},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009ApJ...705..199B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Hu2015,
   title={SUPERMASSIVE BLACK HOLES WITH HIGH ACCRETION RATES IN ACTIVE GALACTIC NUCLEI. III. DETECTION OF Fe ii REVERBERATION IN NINE NARROW-LINE SEYFERT 1 GALAXIES},
   volume={804},
   ISSN={1538-4357},
   url={http://dx.doi.org/10.1088/0004-637X/804/2/138},
   DOI={10.1088/0004-637x/804/2/138},
   number={2},
   journal={The Astrophysical Journal},
   publisher={American Astronomical Society},
   author={Hu, Chen and Du, Pu and Lu, Kai-Xing and Li, Yan-Rong and Wang, Fang and Qiu, Jie and Bai, Jin-Ming and Kaspi, Shai and Ho, Luis C. and Netzer, Hagai and et al.},
   year={2015},
   month={May},
   pages={138}
}
@ARTICLE{2003ApJ...596L..27K,
       author = {{King}, Andrew},
        title = "{Black Holes, Galaxy Formation, and the M$_{BH}$-{\ensuremath{\sigma}} Relation}",
      journal = {\apjl},
     keywords = {Accretion, Accretion Disks, Black Hole Physics, Galaxies: Formation, Galaxies: Nuclei, Galaxies: Quasars: General, Astrophysics},
         year = 2003,
        month = oct,
       volume = {596},
       number = {1},
        pages = {L27-L29},
          doi = {10.1086/379143},
archivePrefix = {arXiv},
       eprint = {astro-ph/0308342},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003ApJ...596L..27K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2013ApJ...769...51Z,
       author = {{Zubovas}, Kastytis and {King}, Andrew},
        title = "{BAL QSOs and Extreme UFOs: The Eddington Connection}",
      journal = {\apj},
     keywords = {accretion, accretion disks, black hole physics, galaxies: evolution, quasars: general, Astrophysics - Astrophysics of Galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2013,
        month = may,
       volume = {769},
       number = {1},
          eid = {51},
        pages = {51},
          doi = {10.1088/0004-637X/769/1/51},
archivePrefix = {arXiv},
       eprint = {1304.1691},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJ...769...51Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{1916MNRAS..77...16E,
       author = {{Eddington}, A.~S.},
        title = "{On the radiative equilibrium of the stars}",
      journal = {\mnras},
         year = 1916,
        month = nov,
       volume = {77},
        pages = {16-35},
          doi = {10.1093/mnras/77.1.16},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1916MNRAS..77...16E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{dinosaur,
       author = {{Tortosa}, Alessia and {Ricci}, Claudio and {Tombesi}, Francesco and {Ho}, Luis C. and {Du}, Pu and {Inayoshi}, Kohei and {Wang}, Jian-Min and {Shangguan}, Jinyi and {Li}, Ruancun},
        title = "{The extreme properties of the nearby hyper-Eddington accreting active galactic nucleus in IRAS 04416+1215}",
      journal = {\mnras},
     keywords = {accretion, accretion discs, black hole physics, galaxies: active, galaxies: nuclei, galaxies: Seyfert, X-rays: galaxies, Astrophysics - Astrophysics of Galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2022,
        month = jan,
       volume = {509},
       number = {3},
        pages = {3599-3615},
          doi = {10.1093/mnras/stab3152},
archivePrefix = {arXiv},
       eprint = {2109.02573},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022MNRAS.509.3599T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2018ApJ...864L..27F,
       author = {{Fukumura}, Keigo and {Kazanas}, Demosthenes and {Shrader}, Chris and {Behar}, Ehud and {Tombesi}, Francesco and {Contopoulos}, Ioannis},
        title = "{Variable Nature of Magnetically Driven Ultra-fast Outflows}",
      journal = {\apjl},
     keywords = {accretion, accretion disks, galaxies: individual: PDS 456, magnetohydrodynamics: MHD, methods: numerical, quasars: absorption lines, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2018,
        month = sep,
       volume = {864},
       number = {2},
          eid = {L27},
        pages = {L27},
          doi = {10.3847/2041-8213/aadd10},
archivePrefix = {arXiv},
       eprint = {1808.08935},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJ...864L..27F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2014ApJ...787...83M,
       author = {{Marinucci}, A. and {Matt}, G. and {Miniutti}, G. and {Guainazzi}, M. and {Parker}, M.~L. and {Brenneman}, L. and {Fabian}, A.~C. and {Kara}, E. and {Arevalo}, P. and {Ballantyne}, D.~R. and {Boggs}, S.~E. and {Cappi}, M. and {Christensen}, F.~E. and {Craig}, W.~W. and {Elvis}, M. and {Hailey}, C.~J. and {Harrison}, F.~A. and {Reynolds}, C.~S. and {Risaliti}, G. and {Stern}, D.~K. and {Walton}, D.~J. and {Zhang}, W.},
        title = "{The Broadband Spectral Variability of MCG-6-30-15 Observed by NuSTAR and XMM-Newton}",
      journal = {\apj},
     keywords = {accretion, accretion disks, galaxies: active, galaxies: Seyfert, X-rays: individual: MCG{\textendash}6-30-015, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2014,
        month = may,
       volume = {787},
       number = {1},
          eid = {83},
        pages = {83},
          doi = {10.1088/0004-637X/787/1/83},
archivePrefix = {arXiv},
       eprint = {1404.3561},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...787...83M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Picomcelli2004,
       author = {{Piconcelli}, E. and {Jimenez-Bail{\'o}n}, E. and {Guainazzi}, M. and {Schartel}, N. and {Rodr{\'\i}guez-Pascual}, P.~M. and {Santos-Lle{\'o}}, M.},
        title = "{Evidence for a multizone warm absorber in the XMM-Newton spectrum of Markarian 304}",
      journal = {\mnras},
     keywords = {galaxies: active, galaxies: individual: Markarian 304, galaxies: Seyfert, X-rays: galaxies, Astrophysics},
         year = 2004,
        month = jun,
       volume = {351},
       number = {1},
        pages = {161-168},
          doi = {10.1111/j.1365-2966.2004.07764.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0404263},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004MNRAS.351..161P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2005MNRAS.359.1469M,
       author = {{McHardy}, I.~M. and {Gunn}, K.~F. and {Uttley}, P. and {Goad}, M.~R.},
        title = "{MCG-6-30-15: long time-scale X-ray variability, black hole mass and active galactic nuclei high states}",
      journal = {\mnras},
     keywords = {black hole physics, galaxies: active, galaxies: individual: MCG-6-30-15, X-rays: binaries, X-rays: galaxies, Astrophysics},
         year = 2005,
        month = jun,
       volume = {359},
       number = {4},
        pages = {1469-1480},
          doi = {10.1111/j.1365-2966.2005.08992.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0503100},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005MNRAS.359.1469M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@article{Collin_2004,
   title={Super-Eddington accretion rates in Narrow Line Seyfert 1 galaxies},
   volume={426},
   ISSN={1432-0746},
   url={http://dx.doi.org/10.1051/0004-6361:20040528},
   DOI={10.1051/0004-6361:20040528},
   number={3},
   journal={Astronomy & Astrophysics},
   publisher={EDP Sciences},
   author={Collin, S. and Kawaguchi, T.},
   year={2004},
   month={Oct},
   pages={797–808}
}
@ARTICLE{1994ApJ...435L.125M,
       author = {{Mineshige}, S. and {Takeuchi}, M. and {Nishimori}, H.},
        title = "{Is a Black Hole Accretion Disk in a Self-organized Critical State?}",
      journal = {\apjl},
     keywords = {Accretion Disks, Black Holes (Astronomy), Galactic Nuclei, Seyfert Galaxies, Stellar Mass Accretion, X Ray Stars, Mathematical Models, Neutron Stars, Power Spectra, Satellite-Borne Instruments, Three Dimensional Motion, X Ray Spectra, Astrophysics, ACCRETION, ACCRETION DISKS, BLACK HOLE PHYSICS, GALAXIES: SEYFERT, X-RAYS: STARS},
         year = 1994,
        month = nov,
       volume = {435},
        pages = {L125},
          doi = {10.1086/187610},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1994ApJ...435L.125M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2003MNRAS.345.1271V,
       author = {{Vaughan}, S. and {Edelson}, R. and {Warwick}, R.~S. and {Uttley}, P.},
        title = "{On characterizing the variability properties of X-ray light curves from active galaxies}",
      journal = {\mnras},
     keywords = {methods: data analysis, galaxies: active, galaxies: individual: Mrk 766, galaxies: Seyfert, X-rays: galaxies, Astrophysics},
         year = 2003,
        month = nov,
       volume = {345},
       number = {4},
        pages = {1271-1284},
          doi = {10.1046/j.1365-2966.2003.07042.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0307420},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003MNRAS.345.1271V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{1994MNRAS.267..974N,
       author = {{Nandra}, K. and {George}, I.~M.},
        title = "{X-ray reprocessing by cold clouds in active galactic nuclei.}",
      journal = {\mnras},
         year = 1994,
        month = apr,
       volume = {267},
        pages = {974-980},
          doi = {10.1093/mnras/267.4.974},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1994MNRAS.267..974N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{1997ApJ...476...70N,
       author = {{Nandra}, K. and {George}, I.~M. and {Mushotzky}, R.~F. and {Turner}, T.~J. and {Yaqoob}, T.},
        title = "{ASCA Observations of Seyfert 1 Galaxies. I. Data Analysis, Imaging, and Timing}",
      journal = {\apj},
     keywords = {Galaxies: Active, Galaxies: Nuclei, Galaxies: Seyfert, X-Rays: Galaxies},
         year = 1997,
        month = feb,
       volume = {476},
       number = {1},
        pages = {70-82},
          doi = {10.1086/303600},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1997ApJ...476...70N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2002ApJ...568..610E,
       author = {{Edelson}, Rick and {Turner}, T.~J. and {Pounds}, Ken and {Vaughan}, Simon and {Markowitz}, Alex and {Marshall}, Herman and {Dobbie}, Paul and {Warwick}, Robert},
        title = "{X-Ray Spectral Variability and Rapid Variability of the Soft X-Ray Spectrum Seyfert 1 Galaxies Arakelian 564 and Ton S180}",
      journal = {\apj},
     keywords = {Galaxies: Active, Galaxies: Individual: Name: Arakelian 564, Galaxies: Individual: Name: Ton S180, Galaxies: Seyfert, X-Rays: Galaxies, Astrophysics},
         year = 2002,
        month = apr,
       volume = {568},
       number = {2},
        pages = {610-626},
          doi = {10.1086/323779},
archivePrefix = {arXiv},
       eprint = {astro-ph/0108387},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2002ApJ...568..610E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2002A&A...388..771C,
       author = {{Collin}, S. and {Boisson}, C. and {Mouchet}, M. and {Dumont}, A. -M. and {Coup{\'e}}, S. and {Porquet}, D. and {Rokaki}, E.},
        title = "{Are quasars accreting at super-Eddington rates?}",
      journal = {\aap},
     keywords = {quasars: general, accretion, accretion disks, galaxies: active, Astrophysics},
         year = 2002,
        month = jun,
       volume = {388},
        pages = {771-786},
          doi = {10.1051/0004-6361:20020550},
archivePrefix = {arXiv},
       eprint = {astro-ph/0203439},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2002A&A...388..771C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Madsen2020,
       author = {{Madsen}, Kristin K. and {Grefenstette}, Brian W. and {Pike}, Sean and {Miyasaka}, Hiromasa and {Brightman}, Murray and {Forster}, Karl and {Harrison}, Fiona A.},
        title = "{NuSTAR low energy effective area correction due to thermal blanket tear}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2020,
        month = may,
          eid = {arXiv:2005.00569},
        pages = {arXiv:2005.00569},
archivePrefix = {arXiv},
       eprint = {2005.00569},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020arXiv200500569M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Luminari2020,
       author = {{Luminari}, A. and {Tombesi}, F. and {Piconcelli}, E. and {Nicastro}, F. and {Fukumura}, K. and {Kazanas}, D. and {Fiore}, F. and {Zappacosta}, L.},
        title = "{The importance of special relativistic effects in modelling ultra-fast outflows}",
      journal = {\aap},
     keywords = {line: profiles, opacity, radiative transfer, relativistic processes, quasars: absorption lines, accretion, accretion disks, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2020,
        month = jan,
       volume = {633},
          eid = {A55},
        pages = {A55},
          doi = {10.1051/0004-6361/201936797},
archivePrefix = {arXiv},
       eprint = {1912.00494},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020A&A...633A..55L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Luminari2021,
       author = {{Luminari}, A. and {Nicastro}, F. and {Elvis}, M. and {Piconcelli}, E. and {Tombesi}, F. and {Zappacosta}, L. and {Fiore}, F.},
        title = "{Speed limits for radiation-driven SMBH winds}",
      journal = {\aap},
     keywords = {accretion, accretion disks, black hole physics, quasars: supermassive black holes, quasars: absorption lines, opacity, relativistic processes, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Astrophysics of Galaxies},
         year = 2021,
        month = feb,
       volume = {646},
          eid = {A111},
        pages = {A111},
          doi = {10.1051/0004-6361/202039396},
archivePrefix = {arXiv},
       eprint = {2012.07877},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021A&A...646A.111L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2017MNRAS.470..800T,
       author = {{Trakhtenbrot}, Benny and {Ricci}, Claudio and {Koss}, Michael J. and {Schawinski}, Kevin and {Mushotzky}, Richard and {Ueda}, Yoshihiro and {Veilleux}, Sylvain and {Lamperti}, Isabella and {Oh}, Kyuseok and {Treister}, Ezequiel and {Stern}, Daniel and {Harrison}, Fiona and {Balokovi{\'c}}, Mislav and {Gehrels}, Neil},
        title = "{BAT AGN Spectroscopic Survey (BASS) - VI. The {\ensuremath{\Gamma}}$_{X}$-L/L$_{Edd}$ relation}",
      journal = {\mnras},
     keywords = {black hole physics, galaxies: active, quasars: general, X-rays: galaxies, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2017,
        month = sep,
       volume = {470},
       number = {1},
        pages = {800-814},
          doi = {10.1093/mnras/stx1117},
archivePrefix = {arXiv},
       eprint = {1705.01550},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017MNRAS.470..800T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{King2015,
       author = {{King}, Andrew and {Pounds}, Ken},
        title = "{Powerful Outflows and Feedback from Active Galactic Nuclei}",
      journal = {\araa},
     keywords = {Astrophysics - Astrophysics of Galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2015,
        month = aug,
       volume = {53},
        pages = {115-154},
          doi = {10.1146/annurev-astro-082214-122316},
archivePrefix = {arXiv},
       eprint = {1503.05206},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ARA&A..53..115K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{King2010,
       author = {{King}, A.~R.},
        title = "{AGN have underweight black holes and reach Eddington}",
      journal = {\mnras},
     keywords = {accretion, accretion discs, black hole physics, galaxies: active, galaxies: formation, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2010,
        month = oct,
       volume = {408},
       number = {1},
        pages = {L95-L98},
          doi = {10.1111/j.1745-3933.2010.00938.x},
archivePrefix = {arXiv},
       eprint = {1008.3367},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010MNRAS.408L..95K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@article{King2003,
   title={Black hole winds},
   volume={345},
   ISSN={1365-2966},
   url={http://dx.doi.org/10.1046/j.1365-8711.2003.06980.x},
   DOI={10.1046/j.1365-8711.2003.06980.x},
   number={2},
   journal={Monthly Notices of the Royal Astronomical Society},
   publisher={Oxford University Press (OUP)},
   author={King, A. R. and Pounds, K. A.},
   year={2003},
   month={Oct},
   pages={657–659}
}
@ARTICLE{Ostriker2010,
       author = {{Ostriker}, Jeremiah P. and {Choi}, Ena and {Ciotti}, Luca and {Novak}, Gregory S. and {Proga}, Daniel},
        title = "{Momentum Driving: Which Physical Processes Dominate Active Galactic Nucleus Feedback?}",
      journal = {\apj},
     keywords = {accretion, accretion disks, black hole physics, galaxies: active, galaxies: nuclei, galaxies: starburst, quasars: general, Astrophysics - Astrophysics of Galaxies},
         year = 2010,
        month = oct,
       volume = {722},
       number = {1},
        pages = {642-652},
          doi = {10.1088/0004-637X/722/1/642},
archivePrefix = {arXiv},
       eprint = {1004.2923},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010ApJ...722..642O},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{dimatteo2005,
       author = {{Di Matteo}, Tiziana and {Springel}, Volker and {Hernquist}, Lars},
        title = "{Energy input from quasars regulates the growth and activity of black holes and their host galaxies}",
      journal = {\nat},
     keywords = {Astrophysics},
         year = 2005,
        month = feb,
       volume = {433},
       number = {7026},
        pages = {604-607},
          doi = {10.1038/nature03335},
archivePrefix = {arXiv},
       eprint = {astro-ph/0502199},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005Natur.433..604D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Struder2001,
       author = {{Str{\"u}der}, L. and {Briel}, U. and {Dennerl}, K. and {Hartmann}, R. and {Kendziorra}, E. and {Meidinger}, N. and {Pfeffermann}, E. and {Reppin}, C. and {Aschenbach}, B. and {Bornemann}, W. and {Br{\"a}uninger}, H. and {Burkert}, W. and {Elender}, M. and {Freyberg}, M. and {Haberl}, F. and {Hartner}, G. and {Heuschmann}, F. and {Hippmann}, H. and {Kastelic}, E. and {Kemmer}, S. and {Kettenring}, G. and {Kink}, W. and {Krause}, N. and {M{\"u}ller}, S. and {Oppitz}, A. and {Pietsch}, W. and {Popp}, M. and {Predehl}, P. and {Read}, A. and {Stephan}, K.~H. and {St{\"o}tter}, D. and {Tr{\"u}mper}, J. and {Holl}, P. and {Kemmer}, J. and {Soltau}, H. and {St{\"o}tter}, R. and {Weber}, U. and {Weichert}, U. and {von Zanthier}, C. and {Carathanassis}, D. and {Lutz}, G. and {Richter}, R.~H. and {Solc}, P. and {B{\"o}ttcher}, H. and {Kuster}, M. and {Staubert}, R. and {Abbey}, A. and {Holland}, A. and {Turner}, M. and {Balasini}, M. and {Bignami}, G.~F. and {La Palombara}, N. and {Villa}, G. and {Buttler}, W. and {Gianini}, F. and {Lain{\'e}}, R. and {Lumb}, D. and {Dhez}, P.},
        title = "{The European Photon Imaging Camera on XMM-Newton: The pn-CCD camera}",
      journal = {\aap},
     keywords = {XMM-NEWTON, BACK ILLUMINATED PN-CCDS, RADIATION HARDNESS, ENERGY RESOLUTION, QUANTUM EFFICIENCY, PARTICLE AND FLOURESCENCE BACKGROUND},
         year = 2001,
        month = jan,
       volume = {365},
        pages = {L18-L26},
          doi = {10.1051/0004-6361:20000066},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001A&A...365L..18S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Debuhr2011,
       author = {{Debuhr}, Jackson and {Quataert}, Eliot and {Ma}, Chung-Pei},
        title = "{The growth of massive black holes in galaxy merger simulations with feedback by radiation pressure}",
      journal = {\mnras},
     keywords = {galaxies: active, galaxies: evolution, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2011,
        month = apr,
       volume = {412},
       number = {2},
        pages = {1341-1360},
          doi = {10.1111/j.1365-2966.2010.17992.x},
archivePrefix = {arXiv},
       eprint = {1006.3312},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011MNRAS.412.1341D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Zubovas2012,
       author = {{Zubovas}, Kastytis and {King}, Andrew},
        title = "{Clearing Out a Galaxy}",
      journal = {\apjl},
     keywords = {accretion, accretion disks, black hole physics, galaxies: evolution, quasars: general, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2012,
        month = feb,
       volume = {745},
       number = {2},
          eid = {L34},
        pages = {L34},
          doi = {10.1088/2041-8205/745/2/L34},
archivePrefix = {arXiv},
       eprint = {1201.0866},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ApJ...745L..34Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Chartas2003,
       author = {{Chartas}, G. and {Brandt}, W.~N. and {Gallagher}, S.~C.},
        title = "{XMM-Newton Reveals the Quasar Outflow in PG 1115+080}",
      journal = {\apj},
     keywords = {Galaxies: Active, Cosmology: Gravitational Lensing, Galaxies: Quasars: Absorption Lines, Galaxies: Quasars: Individual: Alphanumeric: PG 1115+080, Galaxies: Quasars: Individual: Alphanumeric: APM 08279+5255, X-Rays: Galaxies, Astrophysics},
         year = 2003,
        month = sep,
       volume = {595},
       number = {1},
        pages = {85-93},
          doi = {10.1086/377299},
archivePrefix = {arXiv},
       eprint = {astro-ph/0306125},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003ApJ...595...85C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2011ApJ...728...98D,
       author = {{Davis}, Shane W. and {Laor}, Ari},
        title = "{The Radiative Efficiency of Accretion Flows in Individual Active Galactic Nuclei}",
      journal = {\apj},
     keywords = {accretion, accretion disks, black hole physics, galaxies: active, quasars: general, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2011,
        month = feb,
       volume = {728},
       number = {2},
          eid = {98},
        pages = {98},
          doi = {10.1088/0004-637X/728/2/98},
archivePrefix = {arXiv},
       eprint = {1012.3213},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011ApJ...728...98D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{EPIC,
       author = {{Str{\"u}der}, L. and {Briel}, U. and {Dennerl}, K. and {Hartmann}, R. and {Kendziorra}, E. and {Meidinger}, N. and {Pfeffermann}, E. and {Reppin}, C. and {Aschenbach}, B. and {Bornemann}, W. and {Br{\"a}uninger}, H. and {Burkert}, W. and {Elender}, M. and {Freyberg}, M. and {Haberl}, F. and {Hartner}, G. and {Heuschmann}, F. and {Hippmann}, H. and {Kastelic}, E. and {Kemmer}, S. and {Kettenring}, G. and {Kink}, W. and {Krause}, N. and {M{\"u}ller}, S. and {Oppitz}, A. and {Pietsch}, W. and {Popp}, M. and {Predehl}, P. and {Read}, A. and {Stephan}, K.~H. and {St{\"o}tter}, D. and {Tr{\"u}mper}, J. and {Holl}, P. and {Kemmer}, J. and {Soltau}, H. and {St{\"o}tter}, R. and {Weber}, U. and {Weichert}, U. and {von Zanthier}, C. and {Carathanassis}, D. and {Lutz}, G. and {Richter}, R.~H. and {Solc}, P. and {B{\"o}ttcher}, H. and {Kuster}, M. and {Staubert}, R. and {Abbey}, A. and {Holland}, A. and {Turner}, M. and {Balasini}, M. and {Bignami}, G.~F. and {La Palombara}, N. and {Villa}, G. and {Buttler}, W. and {Gianini}, F. and {Lain{\'e}}, R. and {Lumb}, D. and {Dhez}, P.},
        title = "{The European Photon Imaging Camera on XMM-Newton: The pn-CCD camera}",
      journal = {\aap},
     keywords = {XMM-NEWTON, BACK ILLUMINATED PN-CCDS, RADIATION HARDNESS, ENERGY RESOLUTION, QUANTUM EFFICIENCY, PARTICLE AND FLOURESCENCE BACKGROUND},
         year = 2001,
        month = jan,
       volume = {365},
        pages = {L18-L26},
          doi = {10.1051/0004-6361:20000066},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001A&A...365L..18S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@MISC{Lanzuisi2012,
       author = {{Lanzuisi}, Giorgio},
        title = "{Probing the variable, relativistic wind in the high-z QSO HS 1700+6416}",
     keywords = {Active Galactic Nuclei, Quasars, BL-Lac Objects, X-ray Background, HS 1700+6416, HS 1700+6416, HS 1700+6416},
 howpublished = {XMM-Newton Proposal},
         year = 2012,
        month = oct,
        pages = {126},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012xmm..prop..126L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Vignali2015,
       author = {{Vignali}, C. and {Iwasawa}, K. and {Comastri}, A. and {Gilli}, R. and {Lanzuisi}, G. and {Ranalli}, P. and {Cappelluti}, N. and {Mainieri}, V. and {Georgantopoulos}, I. and {Carrera}, F.~J. and {Fritz}, J. and {Brusa}, M. and {Brandt}, W.~N. and {Bauer}, F.~E. and {Fiore}, F. and {Tombesi}, F.},
        title = "{An X-ray outflow in a luminous obscured quasar at z=1.6 in the Chandra Deep-Field South}",
    booktitle = {Demographics and Environment of AGN from Multi-Wavelength Surveys},
         year = 2015,
       editor = {{Georgantopoulos}, Ioannis},
        month = sep,
          eid = {108},
        pages = {108},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015deam.confE.108V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{NuSTAR,
       author = {{Harrison}, Fiona A. and {Craig}, William W. and {Christensen}, Finn E. and {Hailey}, Charles J. and {Zhang}, William W. and {Boggs}, Steven E. and {Stern}, Daniel and {Cook}, W. Rick and {Forster}, Karl and {Giommi}, Paolo and {Grefenstette}, Brian W. and {Kim}, Yunjin and {Kitaguchi}, Takao and {Koglin}, Jason E. and {Madsen}, Kristin K. and {Mao}, Peter H. and {Miyasaka}, Hiromasa and {Mori}, Kaya and {Perri}, Matteo and {Pivovaroff}, Michael J. and {Puccetti}, Simonetta and {Rana}, Vikram R. and {Westergaard}, Niels J. and {Willis}, Jason and {Zoglauer}, Andreas and {An}, Hongjun and {Bachetti}, Matteo and {Barri{\`e}re}, Nicolas M. and {Bellm}, Eric C. and {Bhalerao}, Varun and {Brejnholt}, Nicolai F. and {Fuerst}, Felix and {Liebe}, Carl C. and {Markwardt}, Craig B. and {Nynka}, Melania and {Vogel}, Julia K. and {Walton}, Dominic J. and {Wik}, Daniel R. and {Alexander}, David M. and {Cominsky}, Lynn R. and {Hornschemeier}, Ann E. and {Hornstrup}, Allan and {Kaspi}, Victoria M. and {Madejski}, Greg M. and {Matt}, Giorgio and {Molendi}, Silvano and {Smith}, David M. and {Tomsick}, John A. and {Ajello}, Marco and {Ballantyne}, David R. and {Balokovi{\'c}}, Mislav and {Barret}, Didier and {Bauer}, Franz E. and {Blandford}, Roger D. and {Brandt}, W. Niel and {Brenneman}, Laura W. and {Chiang}, James and {Chakrabarty}, Deepto and {Chenevez}, Jerome and {Comastri}, Andrea and {Dufour}, Francois and {Elvis}, Martin and {Fabian}, Andrew C. and {Farrah}, Duncan and {Fryer}, Chris L. and {Gotthelf}, Eric V. and {Grindlay}, Jonathan E. and {Helfand}, David J. and {Krivonos}, Roman and {Meier}, David L. and {Miller}, Jon M. and {Natalucci}, Lorenzo and {Ogle}, Patrick and {Ofek}, Eran O. and {Ptak}, Andrew and {Reynolds}, Stephen P. and {Rigby}, Jane R. and {Tagliaferri}, Gianpiero and {Thorsett}, Stephen E. and {Treister}, Ezequiel and {Urry}, C. Megan},
        title = "{The Nuclear Spectroscopic Telescope Array (NuSTAR) High-energy X-Ray Mission}",
      journal = {\apj},
     keywords = {space vehicles: instruments, X-rays: general, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2013,
        month = jun,
       volume = {770},
       number = {2},
          eid = {103},
        pages = {103},
          doi = {10.1088/0004-637X/770/2/103},
archivePrefix = {arXiv},
       eprint = {1301.7307},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJ...770..103H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lanzuisi2016,
       author = {{Lanzuisi}, G. and {Perna}, M. and {Comastri}, A. and {Cappi}, M. and {Dadina}, M. and {Marinucci}, A. and {Masini}, A. and {Matt}, G. and {Vagnetti}, F. and {Vignali}, C. and {Ballantyne}, D.~R. and {Bauer}, F.~E. and {Boggs}, S.~E. and {Brandt}, W.~N. and {Brusa}, M. and {Christensen}, F.~E. and {Craig}, W.~W. and {Fabian}, A.~C. and {Farrah}, D. and {Hailey}, C.~J. and {Harrison}, F.~A. and {Luo}, B. and {Piconcelli}, E. and {Puccetti}, S. and {Ricci}, C. and {Saez}, C. and {Stern}, D. and {Walton}, D.~J. and {Zhang}, W.~W.},
        title = "{NuSTAR reveals the extreme properties of the super-Eddington accreting supermassive black hole in PG 1247+267}",
      journal = {\aap},
     keywords = {galaxies: active, galaxies: nuclei, quasars: individual: PG 1247+267, accretion, accretion disks, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2016,
        month = may,
       volume = {590},
          eid = {A77},
        pages = {A77},
          doi = {10.1051/0004-6361/201628325},
archivePrefix = {arXiv},
       eprint = {1604.02462},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016A&A...590A..77L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{XRT,
       author = {{Burrows}, David N. and {Hill}, J.~E. and {Nousek}, J.~A. and {Kennea}, J.~A. and {Wells}, A. and {Osborne}, J.~P. and {Abbey}, A.~F. and {Beardmore}, A. and {Mukerjee}, K. and {Short}, A.~D.~T. and {Chincarini}, G. and {Campana}, S. and {Citterio}, O. and {Moretti}, A. and {Pagani}, C. and {Tagliaferri}, G. and {Giommi}, P. and {Capalbi}, M. and {Tamburelli}, F. and {Angelini}, L. and {Cusumano}, G. and {Br{\"a}uninger}, H.~W. and {Burkert}, W. and {Hartner}, G.~D.},
        title = "{The Swift X-Ray Telescope}",
      journal = {\ssr},
     keywords = {gamma-ray burst, X-ray telescope, Swift, X-ray instrumentation, X-ray CCD detector, X-ray mirrors, {\ensuremath{\gamma}}-ray burst, Astrophysics},
         year = 2005,
        month = oct,
       volume = {120},
       number = {3-4},
        pages = {165-195},
          doi = {10.1007/s11214-005-5097-2},
archivePrefix = {arXiv},
       eprint = {astro-ph/0508071},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005SSRv..120..165B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Ballantyne2011,
       author = {{Ballantyne}, D.~R. and {McDuffie}, J.~R. and {Rusin}, J.~S.},
        title = "{A Correlation between the Ionization State of the Inner Accretion Disk and the Eddington Ratio of Active Galactic Nuclei}",
      journal = {\apj},
     keywords = {accretion, accretion disks, black hole physics, galaxies: active, galaxies: nuclei, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2011,
        month = jun,
       volume = {734},
       number = {2},
          eid = {112},
        pages = {112},
          doi = {10.1088/0004-637X/734/2/112},
archivePrefix = {arXiv},
       eprint = {1104.1984},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011ApJ...734..112B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Blustin2005,
       author = {{Blustin}, A.~J. and {Page}, M.~J. and {Fuerst}, S.~V. and {Branduardi-Raymont}, G. and {Ashton}, C.~E.},
        title = "{The nature and origin of Seyfert warm absorbers}",
      journal = {\aap},
     keywords = {Galaxies: active, X-rays: galaxies, galaxies: general, galaxies: Seyfert, quasars: absorption lines, techniques: spectroscopic, Astrophysics},
         year = 2005,
        month = feb,
       volume = {431},
        pages = {111-125},
          doi = {10.1051/0004-6361:20041775},
archivePrefix = {arXiv},
       eprint = {astro-ph/0411297},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005A&A...431..111B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Kawamuro2016,
       author = {{Kawamuro}, Taiki and {Ueda}, Yoshihiro and {Tazaki}, Fumie and {Ricci}, Claudio and {Terashima}, Yuichi},
        title = "{Suzaku Observations of Moderately Obscured (Compton-thin) Active Galactic Nuclei Selected by Swift/BAT Hard X-ray Survey}",
      journal = {\apjs},
     keywords = {galaxies: active, galaxies: nuclei, X-rays: galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2016,
        month = jul,
       volume = {225},
       number = {1},
          eid = {14},
        pages = {14},
          doi = {10.3847/0067-0049/225/1/14},
archivePrefix = {arXiv},
       eprint = {1606.04941},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ApJS..225...14K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Brandt1997,
       author = {{Brandt}, W.~N. and {Mathur}, S. and {Elvis}, M.},
        title = "{A comparison of the hard ASCA spectral slopes of broad- and narrow-line Seyfert 1 galaxies}",
      journal = {\mnras},
     keywords = {GALAXIES: ACTIVE, X-RAYS: GALAXIES, Astrophysics},
         year = 1997,
        month = mar,
       volume = {285},
       number = {3},
        pages = {L25-L30},
          doi = {10.1093/mnras/285.3.L25},
archivePrefix = {arXiv},
       eprint = {astro-ph/9703100},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1997MNRAS.285L..25B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Shemmer2008,
       author = {{Shemmer}, Ohad and {Brandt}, W.~N. and {Netzer}, Hagai and {Maiolino}, Roberto and {Kaspi}, Shai},
        title = "{The Hard X-Ray Spectrum as a Probe for Black Hole Growth in Radio-Quiet Active Galactic Nuclei}",
      journal = {\apj},
     keywords = {galaxies: active, galaxies: nuclei, quasars: emission lines, X-rays: galaxies, Astrophysics},
         year = 2008,
        month = jul,
       volume = {682},
       number = {1},
        pages = {81-93},
          doi = {10.1086/588776},
archivePrefix = {arXiv},
       eprint = {0804.0803},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008ApJ...682...81S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Shemmer2006,
       author = {{Shemmer}, Ohad and {Brandt}, W.~N. and {Netzer}, Hagai and {Maiolino}, Roberto and {Kaspi}, Shai},
        title = "{The Hard X-Ray Spectral Slope as an Accretion Rate Indicator in Radio-quiet Active Galactic Nuclei}",
      journal = {\apjl},
     keywords = {Galaxies: Active, Galaxies: Nuclei, Galaxies: Quasars: Emission Lines, quasars: individual (Q1346-036), Galaxies: Quasars: Individual: Alphanumeric: HE 2217-2818, X-Rays: Galaxies, Astrophysics},
         year = 2006,
        month = jul,
       volume = {646},
       number = {1},
        pages = {L29-L32},
          doi = {10.1086/506911},
archivePrefix = {arXiv},
       eprint = {astro-ph/0606389},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006ApJ...646L..29S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{1993ApJ...413L..15I,
       author = {{Iwasawa}, Kazushi and {Taniguchi}, Yoshiaki},
        title = "{The X-Ray Baldwin Effect}",
      journal = {\apjl},
     keywords = {Active Galactic Nuclei, Quasars, Seyfert Galaxies, X Ray Spectra, X Rays, Continuous Spectra, Emission Spectra, Ginga Satellite, Spaceborne Astronomy, Spectral Line Width, Astrophysics, GALAXIES: SEYFERT, GALAXIES: QUASARS: EMISSION LINES, X-RAYS: GALAXIES},
         year = 1993,
        month = aug,
       volume = {413},
        pages = {L15},
          doi = {10.1086/186948},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1993ApJ...413L..15I},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1977ApJ...214..679B,
       author = {{Baldwin}, Jack A.},
        title = "{Luminosity Indicators in the Spectra of Quasi-Stellar Objects}",
      journal = {\apj},
         year = 1977,
        month = jun,
       volume = {214},
        pages = {679-684},
          doi = {10.1086/155294},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1977ApJ...214..679B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Risaliti2009,
       author = {{Risaliti}, G. and {Young}, M. and {Elvis}, M.},
        title = "{The Sloan Digital Sky Survey/XMM-Newton Quasar Survey: Correlation Between X-Ray Spectral Slope and Eddington Ratio}",
      journal = {\apjl},
     keywords = {galaxies: active, X-rays: galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2009,
        month = jul,
       volume = {700},
       number = {1},
        pages = {L6-L10},
          doi = {10.1088/0004-637X/700/1/L6},
archivePrefix = {arXiv},
       eprint = {0906.1983},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009ApJ...700L...6R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Lanzuisi2019,
       author = {{Lanzuisi}, G. and {Gilli}, R. and {Cappi}, M. and {Dadina}, M. and {Bianchi}, S. and {Brusa}, M. and {Chartas}, G. and {Civano}, F. and {Comastri}, A. and {Marinucci}, A. and {Middei}, R. and {Piconcelli}, E. and {Vignali}, C. and {Brandt}, W.~N. and {Tombesi}, F. and {Gaspari}, M.},
        title = "{NuSTAR Measurement of Coronal Temperature in Two Luminous, High-redshift Quasars}",
      journal = {\apjl},
     keywords = {accretion, accretion disks, black hole physics, X-rays: galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2019,
        month = apr,
       volume = {875},
       number = {2},
          eid = {L20},
        pages = {L20},
          doi = {10.3847/2041-8213/ab15dc},
archivePrefix = {arXiv},
       eprint = {1904.04784},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...875L..20L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@misc{liu2021observational,
      title={On the Observational Difference Between the Accretion Disk-Corona Connections among Super- and Sub-Eddington Accreting Active Galactic Nuclei}, 
      author={Hezhen Liu and B. Luo and W. N. Brandt and Michael S. Brotherton and S. C. Gallagher and Q. Ni and Ohad Shemmer and J. D. Timlin III au2},
      year={2021},
      eprint={2102.02832},
      archivePrefix={arXiv},
      primaryClass={astro-ph.GA}
}
@ARTICLE{Brightman2013,
       author = {{Brightman}, M. and {Silverman}, J.~D. and {Mainieri}, V. and {Ueda}, Y. and {Schramm}, M. and {Matsuoka}, K. and {Nagao}, T. and {Steinhardt}, C. and {Kartaltepe}, J. and {Sanders}, D.~B. and {Treister}, E. and {Shemmer}, O. and {Brandt}, W.~N. and {Brusa}, M. and {Comastri}, A. and {Ho}, L.~C. and {Lanzuisi}, G. and {Lusso}, E. and {Nandra}, K. and {Salvato}, M. and {Zamorani}, G. and {Akiyama}, M. and {Alexander}, D.~M. and {Bongiorno}, A. and {Capak}, P. and {Civano}, F. and {Del Moro}, A. and {Doi}, A. and {Elvis}, M. and {Hasinger}, G. and {Laird}, E.~S. and {Masters}, D. and {Mignoli}, M. and {Ohta}, K. and {Schawinski}, K. and {Taniguchi}, Y.},
        title = "{A statistical relation between the X-ray spectral index and Eddington ratio of active galactic nuclei in deep surveys}",
      journal = {\mnras},
     keywords = {accretion, accretion discs, galaxies: active, galaxies: nuclei, quasars: emission lines, quasars: general, X-rays: galaxies, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2013,
        month = aug,
       volume = {433},
       number = {3},
        pages = {2485-2496},
          doi = {10.1093/mnras/stt920},
archivePrefix = {arXiv},
       eprint = {1305.3917},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013MNRAS.433.2485B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Guainazzi2006,
       author = {{Guainazzi}, M. and {Siemiginowska}, A. and {Stanghellini}, C. and {Grandi}, P. and {Piconcelli}, E. and {Azubike Ugwoke}, C.},
        title = "{A hard X-ray view of giga-hertz peaked spectrum radio galaxies}",
      journal = {\aap},
     keywords = {galaxies: jets, galaxies: quasars: individual: COINSJ0029+3456, PKS 0500+019, PKS 0941-080, PKS2128+048, X-ray: galaxies, Astrophysics},
         year = 2006,
        month = jan,
       volume = {446},
       number = {1},
        pages = {87-96},
          doi = {10.1051/0004-6361:20053374},
archivePrefix = {arXiv},
       eprint = {astro-ph/0509043},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006A&A...446...87G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2016ApJS..225...14K,
       author = {{Kawamuro}, Taiki and {Ueda}, Yoshihiro and {Tazaki}, Fumie and {Ricci}, Claudio and {Terashima}, Yuichi},
        title = "{Suzaku Observations of Moderately Obscured (Compton-thin) Active Galactic Nuclei Selected by Swift/BAT Hard X-ray Survey}",
      journal = {\apjs},
     keywords = {galaxies: active, galaxies: nuclei, X-rays: galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2016,
        month = jul,
       volume = {225},
       number = {1},
          eid = {14},
        pages = {14},
          doi = {10.3847/0067-0049/225/1/14},
archivePrefix = {arXiv},
       eprint = {1606.04941},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ApJS..225...14K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2016ApJ...826...93B,
       author = {{Brightman}, M. and {Masini}, A. and {Ballantyne}, D.~R. and {Balokovi{\'c}}, M. and {Brandt}, W.~N. and {Chen}, C. -T. and {Comastri}, A. and {Farrah}, D. and {Gandhi}, P. and {Harrison}, F.~A. and {Ricci}, C. and {Stern}, D. and {Walton}, D.~J.},
        title = "{A Growth-rate Indicator for Compton-thick Active Galactic Nuclei}",
      journal = {\apj},
     keywords = {black hole physics, galaxies: general, galaxies: nuclei, galaxies: Seyfert, masers, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Astrophysics of Galaxies},
         year = 2016,
        month = jul,
       volume = {826},
       number = {1},
          eid = {93},
        pages = {93},
          doi = {10.3847/0004-637X/826/1/93},
archivePrefix = {arXiv},
       eprint = {1606.09265},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ApJ...826...93B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2013MNRAS.433.2485B,
       author = {{Brightman}, M. and {Silverman}, J.~D. and {Mainieri}, V. and {Ueda}, Y. and {Schramm}, M. and {Matsuoka}, K. and {Nagao}, T. and {Steinhardt}, C. and {Kartaltepe}, J. and {Sanders}, D.~B. and {Treister}, E. and {Shemmer}, O. and {Brandt}, W.~N. and {Brusa}, M. and {Comastri}, A. and {Ho}, L.~C. and {Lanzuisi}, G. and {Lusso}, E. and {Nandra}, K. and {Salvato}, M. and {Zamorani}, G. and {Akiyama}, M. and {Alexander}, D.~M. and {Bongiorno}, A. and {Capak}, P. and {Civano}, F. and {Del Moro}, A. and {Doi}, A. and {Elvis}, M. and {Hasinger}, G. and {Laird}, E.~S. and {Masters}, D. and {Mignoli}, M. and {Ohta}, K. and {Schawinski}, K. and {Taniguchi}, Y.},
        title = "{A statistical relation between the X-ray spectral index and Eddington ratio of active galactic nuclei in deep surveys}",
      journal = {\mnras},
     keywords = {accretion, accretion discs, galaxies: active, galaxies: nuclei, quasars: emission lines, quasars: general, X-rays: galaxies, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2013,
        month = aug,
       volume = {433},
       number = {3},
        pages = {2485-2496},
          doi = {10.1093/mnras/stt920},
archivePrefix = {arXiv},
       eprint = {1305.3917},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013MNRAS.433.2485B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013MNRAS.433..648F,
       author = {{Fanali}, R. and {Caccianiga}, A. and {Severgnini}, P. and {Della Ceca}, R. and {Marchese}, E. and {Carrera}, F.~J. and {Corral}, A. and {Mateos}, S.},
        title = "{Studying the relationship between X-ray emission and accretion in AGN using the XMM-Newton Bright Serendipitous Survey}",
      journal = {\mnras},
     keywords = {galaxies: active, galaxies: nuclei, quasars: general, X-rays: galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2013,
        month = jul,
       volume = {433},
       number = {1},
        pages = {648-658},
          doi = {10.1093/mnras/stt757},
archivePrefix = {arXiv},
       eprint = {1305.0564},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013MNRAS.433..648F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2009ApJ...700L...6R,
       author = {{Risaliti}, G. and {Young}, M. and {Elvis}, M.},
        title = "{The Sloan Digital Sky Survey/XMM-Newton Quasar Survey: Correlation Between X-Ray Spectral Slope and Eddington Ratio}",
      journal = {\apjl},
     keywords = {galaxies: active, X-rays: galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2009,
        month = jul,
       volume = {700},
       number = {1},
        pages = {L6-L10},
          doi = {10.1088/0004-637X/700/1/L6},
archivePrefix = {arXiv},
       eprint = {0906.1983},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009ApJ...700L...6R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2008ApJ...682...81S,
       author = {{Shemmer}, Ohad and {Brandt}, W.~N. and {Netzer}, Hagai and {Maiolino}, Roberto and {Kaspi}, Shai},
        title = "{The Hard X-Ray Spectrum as a Probe for Black Hole Growth in Radio-Quiet Active Galactic Nuclei}",
      journal = {\apj},
     keywords = {galaxies: active, galaxies: nuclei, quasars: emission lines, X-rays: galaxies, Astrophysics},
         year = 2008,
        month = jul,
       volume = {682},
       number = {1},
        pages = {81-93},
          doi = {10.1086/588776},
archivePrefix = {arXiv},
       eprint = {0804.0803},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008ApJ...682...81S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2006ApJ...646L..29S,
       author = {{Shemmer}, Ohad and {Brandt}, W.~N. and {Netzer}, Hagai and {Maiolino}, Roberto and {Kaspi}, Shai},
        title = "{The Hard X-Ray Spectral Slope as an Accretion Rate Indicator in Radio-quiet Active Galactic Nuclei}",
      journal = {\apjl},
     keywords = {Galaxies: Active, Galaxies: Nuclei, Galaxies: Quasars: Emission Lines, quasars: individual (Q1346-036), Galaxies: Quasars: Individual: Alphanumeric: HE 2217-2818, X-Rays: Galaxies, Astrophysics},
         year = 2006,
        month = jul,
       volume = {646},
       number = {1},
        pages = {L29-L32},
          doi = {10.1086/506911},
archivePrefix = {arXiv},
       eprint = {astro-ph/0606389},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006ApJ...646L..29S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@INPROCEEDINGS{1997AAS...190.5102B,
       author = {{Brandt}, W.~N. and {Mathur}, S. and {Elvis}, M. and {Boller}, Th.},
        title = "{ASCA observations of ultrasoft narrow-line Seyfert 1 galaxies}",
    booktitle = {American Astronomical Society Meeting Abstracts \#190},
         year = 1997,
       series = {American Astronomical Society Meeting Abstracts},
       volume = {190},
        month = may,
          eid = {51.02},
        pages = {51.02},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1997AAS...190.5102B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Bianchi2009,
       author = {{Bianchi}, S. and {Guainazzi}, M. and {Matt}, G. and {Fonseca Bonilla}, N. and {Ponti}, G.},
        title = "{CAIXA: a catalogue of AGN in the XMM-Newton archive. I. Spectral analysis}",
      journal = {\aap},
     keywords = {galaxies: active, galaxies: Seyfert, quasars: general, X-rays: general, Astrophysics},
         year = 2009,
        month = feb,
       volume = {495},
       number = {2},
        pages = {421-430},
          doi = {10.1051/0004-6361:200810620},
archivePrefix = {arXiv},
       eprint = {0811.1126},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009A&A...495..421B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@article{Ricci_2018,
   title={BAT AGN Spectroscopic Survey – XII. The relation between coronal properties of active galactic nuclei and the Eddington ratio},
   volume={480},
   ISSN={1365-2966},
   url={http://dx.doi.org/10.1093/mnras/sty1879},
   DOI={10.1093/mnras/sty1879},
   number={2},
   journal={Monthly Notices of the Royal Astronomical Society},
   publisher={Oxford University Press (OUP)},
   author={Ricci, C and Ho, L C and Fabian, A C and Trakhtenbrot, B and Koss, M J and Ueda, Y and Lohfink, A and Shimizu, T and Bauer, F E and Mushotzky, R and et al.},
   year={2018},
   month={Jul},
   pages={1819–1830}
}
@ARTICLE{2017MNRAS.466.3161S,
       author = {{Shimizu}, T. Taro and {Mushotzky}, Richard F. and {Mel{\'e}ndez}, Marcio and {Koss}, Michael J. and {Barger}, Amy J. and {Cowie}, Lennox L.},
        title = "{Herschel far-infrared photometry of the Swift Burst Alert Telescope active galactic nuclei sample of the local universe - III. Global star-forming properties and the lack of a connection to nuclear activity}",
      journal = {\mnras},
     keywords = {galaxies: active, galaxies: evolution, galaxies: Seyfert, galaxies: star formation, infrared: galaxies, Astrophysics - Astrophysics of Galaxies},
         year = 2017,
        month = apr,
       volume = {466},
       number = {3},
        pages = {3161-3183},
          doi = {10.1093/mnras/stw3268},
archivePrefix = {arXiv},
       eprint = {1612.03941},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017MNRAS.466.3161S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{1985ApJ...293..192F,
       author = {{Feigelson}, E.~D. and {Nelson}, P.~I.},
        title = "{Statistical methods for astronomical data with upper limits. I. Univariate distributions.}",
      journal = {\apj},
     keywords = {Multivariate Statistical Analysis, Radio Astronomy, X Ray Astronomy, Error Analysis, Galaxies, Maximum Likelihood Estimates, Radio Sources (Astronomy), Astrophysics},
         year = 1985,
        month = jun,
       volume = {293},
        pages = {192-206},
          doi = {10.1086/163225},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1985ApJ...293..192F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@article{Ricci_2017,
   title={BAT AGN Spectroscopic Survey. V. X-Ray Properties of the
                    Swift
                    /BAT 70-month AGN Catalog},
   volume={233},
   ISSN={1538-4365},
   url={http://dx.doi.org/10.3847/1538-4365/aa96ad},
   DOI={10.3847/1538-4365/aa96ad},
   number={2},
   journal={The Astrophysical Journal Supplement Series},
   publisher={American Astronomical Society},
   author={Ricci, C. and Trakhtenbrot, B. and Koss, M. J. and Ueda, Y. and Del Vecchio, I. and Treister, E. and Schawinski, K. and Paltani, S. and Oh, K. and Lamperti, I. and et al.},
   year={2017},
   month={Dec},
   pages={17}
}


@ARTICLE{2014ApJ...796..106J,
       author = {{Jiang}, Yan-Fei and {Stone}, James M. and {Davis}, Shane W.},
        title = "{A Global Three-dimensional Radiation Magneto-hydrodynamic Simulation of Super-Eddington Accretion Disks}",
      journal = {\apj},
     keywords = {accretion, accretion disks, magnetohydrodynamics: MHD, methods: numerical, radiative transfer, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2014,
        month = dec,
       volume = {796},
       number = {2},
          eid = {106},
        pages = {106},
          doi = {10.1088/0004-637X/796/2/106},
archivePrefix = {arXiv},
       eprint = {1410.0678},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...796..106J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Ricci2014,
       author = {{Ricci}, C. and {Ueda}, Y. and {Paltani}, S. and {Ichikawa}, K. and {Gandhi}, P. and {Awaki}, H.},
        title = "{Iron K{\ensuremath{\alpha}} emission in type-I and type-II active galactic nuclei}",
      journal = {\mnras},
     keywords = {galaxies: active, galaxies: nuclei, quasars: general, galaxies: Seyfert, X-rays: diffuse background, X-rays: galaxies, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2014,
        month = jul,
       volume = {441},
       number = {4},
        pages = {3622-3633},
          doi = {10.1093/mnras/stu735},
archivePrefix = {arXiv},
       eprint = {1405.7575},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014MNRAS.441.3622R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2000ApJ...534..718N,
       author = {{Nayakshin}, Sergei},
        title = "{On the X-Ray-heated Skin of Accretion Disks}",
      journal = {\apj},
     keywords = {Accretion, Accretion Disks, Line: Formation, Radiation Mechanisms: Nonthermal, X-Rays: General},
         year = 2000,
        month = may,
       volume = {534},
       number = {2},
        pages = {718-722},
          doi = {10.1086/308801},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000ApJ...534..718N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{1997ApJ...488L..91N,
       author = {{Nandra}, K. and {George}, I.~M. and {Mushotzky}, R.~F. and {Turner}, T.~J. and {Yaqoob}, T.},
        title = "{On the Dependence of the Iron K-Line Profiles with Luminosity in Active Galactic Nuclei}",
      journal = {\apjl},
     keywords = {GALAXIES: ACTIVE, GALAXIES: NUCLEI, QUASARS: GENERAL, X-RAYS: GALAXIES, Galaxies: Active, Galaxies: Nuclei, Galaxies: Quasars: General, X-Rays: Galaxies, Astrophysics},
         year = 1997,
        month = oct,
       volume = {488},
       number = {2},
        pages = {L91-L94},
          doi = {10.1086/310937},
archivePrefix = {arXiv},
       eprint = {astro-ph/9708030},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1997ApJ...488L..91N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2006ApJ...644..725J,
       author = {{Jiang}, P. and {Wang}, J.~X. and {Wang}, T.~G.},
        title = "{On the X-Ray Baldwin Effect for Narrow Fe K{\ensuremath{\alpha}} Emission Lines}",
      journal = {\apj},
     keywords = {Galaxies: Active, Galaxies: Quasars: Emission Lines, X-Rays: Galaxies, Astrophysics},
         year = 2006,
        month = jun,
       volume = {644},
       number = {2},
        pages = {725-732},
          doi = {10.1086/503866},
archivePrefix = {arXiv},
       eprint = {astro-ph/0603339},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006ApJ...644..725J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2004MNRAS.347..316P,
       author = {{Page}, K.~L. and {O'Brien}, P.~T. and {Reeves}, J.~N. and {Turner}, M.~J.~L.},
        title = "{An X-ray Baldwin effect for the narrow Fe K{\ensuremath{\alpha}} lines observed in active galactic nuclei}",
      journal = {\mnras},
     keywords = {galaxies: active, quasars: emission lines, X-rays: galaxies, Astrophysics},
         year = 2004,
        month = jan,
       volume = {347},
       number = {1},
        pages = {316-322},
          doi = {10.1111/j.1365-2966.2004.07203.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0309394},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004MNRAS.347..316P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013A&A...549A..72P,
       author = {{Ponti}, G. and {Cappi}, M. and {Costantini}, E. and {Bianchi}, S. and {Kaastra}, J.~S. and {De Marco}, B. and {Fender}, R.~P. and {Petrucci}, P. -O. and {Kriss}, G.~A. and {Steenbrugge}, K.~C. and {Arav}, N. and {Behar}, E. and {Branduardi-Raymont}, G. and {Dadina}, M. and {Ebrero}, J. and {Lubi{\'n}ski}, P. and {Mehdipour}, M. and {Paltani}, S. and {Pinto}, C. and {Tombesi}, F.},
        title = "{Multiwavelength campaign on Mrk 509. XI. Reverberation of the Fe K{\ensuremath{\alpha}} line}",
      journal = {\aap},
     keywords = {accretion, accretion disks, black hole physics, methods: data analysis, galaxies: individual: Mrk 509, galaxies: active, galaxies: Seyfert, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2013,
        month = jan,
       volume = {549},
          eid = {A72},
        pages = {A72},
          doi = {10.1051/0004-6361/201219450},
archivePrefix = {arXiv},
       eprint = {1207.0831},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013A&A...549A..72P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Bianchi2007,
       author = {{Bianchi}, S. and {Guainazzi}, M. and {Matt}, G. and {Fonseca Bonilla}, N.},
        title = "{On the Iwasawa-Taniguchi effect of radio-quiet AGN}",
      journal = {\aap},
     keywords = {galaxies: active, galaxies: Seyfert, quasars: general, X-rays: general, Astrophysics},
         year = 2007,
        month = may,
       volume = {467},
       number = {1},
        pages = {L19-L22},
          doi = {10.1051/0004-6361:20077331},
archivePrefix = {arXiv},
       eprint = {astro-ph/0703433},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007A&A...467L..19B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Shu2010,
       author = {{Shu}, X.~W. and {Yaqoob}, T. and {Wang}, J.~X.},
        title = "{The Cores of the Fe K{\ensuremath{\alpha}} Lines in Active Galactic Nuclei: An Extended Chandra High Energy Grating Sample}",
      journal = {\apjs},
     keywords = {galaxies: active, line: profiles, X-rays: galaxies, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Astrophysics of Galaxies},
         year = 2010,
        month = apr,
       volume = {187},
       number = {2},
        pages = {581-606},
          doi = {10.1088/0067-0049/187/2/581},
archivePrefix = {arXiv},
       eprint = {1003.1790},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010ApJS..187..581S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Fabian_1994,
       author = {{Fabian}, A.~C.},
        title = "{Hot Plasmas and the Generation of Gamma Rays}",
      journal = {\apjs},
     keywords = {Bremsstrahlung, Gamma Rays, High Temperature Plasmas, Pair Production, Space Plasmas, Thermal Plasmas, Active Galactic Nuclei, Black Holes (Astronomy), Compton Effect, Optical Thickness, Thermalization (Energy Absorption), X Ray Spectra, Space Radiation, GAMMA RAYS: THEORY, PLASMAS},
         year = 1994,
        month = jun,
       volume = {92},
        pages = {555},
          doi = {10.1086/192015},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1994ApJS...92..555F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1994ApJ...429L..53G,
       author = {{Ghisellini}, Gabriele and {Haardt}, Francesco},
        title = "{On Thermal Comptonization in E plus or minus Pair Plasmas}",
      journal = {\apjl},
     keywords = {Compton Effect, Electron-Positron Pairs, Gamma Ray Spectra, Plasma Physics, Plasmas (Physics), Seyfert Galaxies, X Ray Spectra, Luminosity, Plasma Equilibrium, Plasma Temperature, Astronomy, RADIATION MECHANISMS: THERMAL, GALAXIES: SEYFERT, GAMMA RAYS: THEORY, PLASMAS, X-RAYS: GENERAL, Astrophysics},
         year = 1994,
        month = jul,
       volume = {429},
        pages = {L53},
          doi = {10.1086/187411},
archivePrefix = {arXiv},
       eprint = {astro-ph/9405055},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1994ApJ...429L..53G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Turner2001,
       author = {{Turner}, M.~J.~L. and {Abbey}, A. and {Arnaud}, M. and {Balasini}, M. and {Barbera}, M. and {Belsole}, E. and {Bennie}, P.~J. and {Bernard}, J.~P. and {Bignami}, G.~F. and {Boer}, M. and {Briel}, U. and {Butler}, I. and {Cara}, C. and {Chabaud}, C. and {Cole}, R. and {Collura}, A. and {Conte}, M. and {Cros}, A. and {Denby}, M. and {Dhez}, P. and {Di Coco}, G. and {Dowson}, J. and {Ferrando}, P. and {Ghizzardi}, S. and {Gianotti}, F. and {Goodall}, C.~V. and {Gretton}, L. and {Griffiths}, R.~G. and {Hainaut}, O. and {Hochedez}, J.~F. and {Holland}, A.~D. and {Jourdain}, E. and {Kendziorra}, E. and {Lagostina}, A. and {Laine}, R. and {La Palombara}, N. and {Lortholary}, M. and {Lumb}, D. and {Marty}, P. and {Molendi}, S. and {Pigot}, C. and {Poindron}, E. and {Pounds}, K.~A. and {Reeves}, J.~N. and {Reppin}, C. and {Rothenflug}, R. and {Salvetat}, P. and {Sauvageot}, J.~L. and {Schmitt}, D. and {Sembay}, S. and {Short}, A.~D.~T. and {Spragg}, J. and {Stephen}, J. and {Str{\"u}der}, L. and {Tiengo}, A. and {Trifoglio}, M. and {Tr{\"u}mper}, J. and {Vercellone}, S. and {Vigroux}, L. and {Villa}, G. and {Ward}, M.~J. and {Whitehead}, S. and {Zonca}, E.},
        title = "{The European Photon Imaging Camera on XMM-Newton: The MOS cameras}",
      journal = {\aap},
     keywords = {INSTRUMENTATION: DETECTORS, X-RAYS: GENERAL, Astrophysics},
         year = 2001,
        month = jan,
       volume = {365},
        pages = {L27-L35},
          doi = {10.1051/0004-6361:20000087},
archivePrefix = {arXiv},
       eprint = {astro-ph/0011498},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001A&A...365L..27T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Jansen2001,
       author = {{Jansen}, F. and {Lumb}, D. and {Altieri}, B. and {Clavel}, J. and {Ehle}, M. and {Erd}, C. and {Gabriel}, C. and {Guainazzi}, M. and {Gondoin}, P. and {Much}, R. and {Munoz}, R. and {Santos}, M. and {Schartel}, N. and {Texier}, D. and {Vacanti}, G.},
        title = "{XMM-Newton observatory. I. The spacecraft and operations}",
      journal = {\aap},
     keywords = {INSTRUMENTS, X-RAY ASTRONOMY},
         year = 2001,
        month = jan,
       volume = {365},
        pages = {L1-L6},
          doi = {10.1051/0004-6361:20000036},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001A&A...365L...1J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{denHerder2001,
       author = {{den Herder}, J.~W. and {Brinkman}, A.~C. and {Kahn}, S.~M. and {Branduardi-Raymont}, G. and {Thomsen}, K. and {Aarts}, H. and {Audard}, M. and {Bixler}, J.~V. and {den Boggende}, A.~J. and {Cottam}, J. and {Decker}, T. and {Dubbeldam}, L. and {Erd}, C. and {Goulooze}, H. and {G{\"u}del}, M. and {Guttridge}, P. and {Hailey}, C.~J. and {Janabi}, K. Al and {Kaastra}, J.~S. and {de Korte}, P.~A.~J. and {van Leeuwen}, B.~J. and {Mauche}, C. and {McCalden}, A.~J. and {Mewe}, R. and {Naber}, A. and {Paerels}, F.~B. and {Peterson}, J.~R. and {Rasmussen}, A.~P. and {Rees}, K. and {Sakelliou}, I. and {Sako}, M. and {Spodek}, J. and {Stern}, M. and {Tamura}, T. and {Tandy}, J. and {de Vries}, C.~P. and {Welch}, S. and {Zehnder}, A.},
        title = "{The Reflection Grating Spectrometer on board XMM-Newton}",
      journal = {\aap},
     keywords = {SPACE VEHICLES: INSTRUMENTS, REFLECTION GRATINGS, \textbackslashTEXTIT\{XMM-NEWTON\}},
         year = 2001,
        month = jan,
       volume = {365},
        pages = {L7-L17},
          doi = {10.1051/0004-6361:20000058},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001A&A...365L...7D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Harrison2013,
       author = {{Harrison}, Fiona A. and {Craig}, William W. and {Christensen}, Finn E. and {Hailey}, Charles J. and {Zhang}, William W. and {Boggs}, Steven E. and {Stern}, Daniel and {Cook}, W. Rick and {Forster}, Karl and {Giommi}, Paolo and {Grefenstette}, Brian W. and {Kim}, Yunjin and {Kitaguchi}, Takao and {Koglin}, Jason E. and {Madsen}, Kristin K. and {Mao}, Peter H. and {Miyasaka}, Hiromasa and {Mori}, Kaya and {Perri}, Matteo and {Pivovaroff}, Michael J. and {Puccetti}, Simonetta and {Rana}, Vikram R. and {Westergaard}, Niels J. and {Willis}, Jason and {Zoglauer}, Andreas and {An}, Hongjun and {Bachetti}, Matteo and {Barri{\`e}re}, Nicolas M. and {Bellm}, Eric C. and {Bhalerao}, Varun and {Brejnholt}, Nicolai F. and {Fuerst}, Felix and {Liebe}, Carl C. and {Markwardt}, Craig B. and {Nynka}, Melania and {Vogel}, Julia K. and {Walton}, Dominic J. and {Wik}, Daniel R. and {Alexander}, David M. and {Cominsky}, Lynn R. and {Hornschemeier}, Ann E. and {Hornstrup}, Allan and {Kaspi}, Victoria M. and {Madejski}, Greg M. and {Matt}, Giorgio and {Molendi}, Silvano and {Smith}, David M. and {Tomsick}, John A. and {Ajello}, Marco and {Ballantyne}, David R. and {Balokovi{\'c}}, Mislav and {Barret}, Didier and {Bauer}, Franz E. and {Blandford}, Roger D. and {Brandt}, W. Niel and {Brenneman}, Laura W. and {Chiang}, James and {Chakrabarty}, Deepto and {Chenevez}, Jerome and {Comastri}, Andrea and {Dufour}, Francois and {Elvis}, Martin and {Fabian}, Andrew C. and {Farrah}, Duncan and {Fryer}, Chris L. and {Gotthelf}, Eric V. and {Grindlay}, Jonathan E. and {Helfand}, David J. and {Krivonos}, Roman and {Meier}, David L. and {Miller}, Jon M. and {Natalucci}, Lorenzo and {Ogle}, Patrick and {Ofek}, Eran O. and {Ptak}, Andrew and {Reynolds}, Stephen P. and {Rigby}, Jane R. and {Tagliaferri}, Gianpiero and {Thorsett}, Stephen E. and {Treister}, Ezequiel and {Urry}, C. Megan},
        title = "{The Nuclear Spectroscopic Telescope Array (NuSTAR) High-energy X-Ray Mission}",
      journal = {\apj},
     keywords = {space vehicles: instruments, X-rays: general, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2013,
        month = jun,
       volume = {770},
       number = {2},
          eid = {103},
        pages = {103},
          doi = {10.1088/0004-637X/770/2/103},
archivePrefix = {arXiv},
       eprint = {1301.7307},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJ...770..103H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Arnaud1996,
       author = {{Arnaud}, K.~A.},
        title = "{XSPEC: The First Ten Years}",
    booktitle = {Astronomical Data Analysis Software and Systems V},
         year = 1996,
       editor = {{Jacoby}, George H. and {Barnes}, Jeannette},
       series = {Astronomical Society of the Pacific Conference Series},
       volume = {101},
        month = jan,
        pages = {17},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1996ASPC..101...17A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{HI4PI2016,
       author = {{HI4PI Collaboration} and {Ben Bekhti}, N. and {Fl{\"o}er}, L. and {Keller}, R. and {Kerp}, J. and {Lenz}, D. and {Winkel}, B. and {Bailin}, J. and {Calabretta}, M.~R. and {Dedes}, L. and {Ford}, H.~A. and {Gibson}, B.~K. and {Haud}, U. and {Janowiecki}, S. and {Kalberla}, P.~M.~W. and {Lockman}, F.~J. and {McClure-Griffiths}, N.~M. and {Murphy}, T. and {Nakanishi}, H. and {Pisano}, D.~J. and {Staveley-Smith}, L.},
        title = "{HI4PI: A full-sky H I survey based on EBHIS and GASS}",
      journal = {\aap},
     keywords = {surveys, ISM: atoms, techniques: spectroscopic, Astrophysics - Astrophysics of Galaxies},
         year = 2016,
        month = oct,
       volume = {594},
          eid = {A116},
        pages = {A116},
          doi = {10.1051/0004-6361/201629178},
archivePrefix = {arXiv},
       eprint = {1610.06175},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016A&A...594A.116H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Madsen2015,
       author = {{Madsen}, Kristin K. and {Harrison}, Fiona A. and {Markwardt}, Craig B. and {An}, Hongjun and {Grefenstette}, Brian W. and {Bachetti}, Matteo and {Miyasaka}, Hiromasa and {Kitaguchi}, Takao and {Bhalerao}, Varun and {Boggs}, Steve and {Christensen}, Finn E. and {Craig}, William W. and {Forster}, Karl and {Fuerst}, Felix and {Hailey}, Charles J. and {Perri}, Matteo and {Puccetti}, Simonetta and {Rana}, Vikram and {Stern}, Daniel and {Walton}, Dominic J. and {J{\o}rgen Westergaard}, Niels and {Zhang}, William W.},
        title = "{Calibration of the NuSTAR High-energy Focusing X-ray Telescope.}",
      journal = {\apjs},
     keywords = {instrumentation: detectors, space vehicles: instruments, telescopes, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2015,
        month = sep,
       volume = {220},
       number = {1},
          eid = {8},
        pages = {8},
          doi = {10.1088/0067-0049/220/1/8},
archivePrefix = {arXiv},
       eprint = {1504.01672},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJS..220....8M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Wilms2000,
       author = {{Wilms}, J. and {Allen}, A. and {McCray}, R.},
        title = "{On the Absorption of X-Rays in the Interstellar Medium}",
      journal = {\apj},
     keywords = {Atomic Data, ISM: Dust, Extinction, ISM: Abundances, X-Rays: ISM, Astrophysics},
         year = 2000,
        month = oct,
       volume = {542},
       number = {2},
        pages = {914-924},
          doi = {10.1086/317016},
archivePrefix = {arXiv},
       eprint = {astro-ph/0008425},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000ApJ...542..914W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Salpeter1964,
       author = {{Salpeter}, E.~E.},
        title = "{Accretion of Interstellar Matter by Massive Objects.}",
      journal = {\apj},
         year = 1964,
        month = aug,
       volume = {140},
        pages = {796-800},
          doi = {10.1086/147973},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1964ApJ...140..796S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Magorrian1998,
       author = {{Magorrian}, John and {Tremaine}, Scott and {Richstone}, Douglas and {Bender}, Ralf and {Bower}, Gary and {Dressler}, Alan and {Faber}, S.~M. and {Gebhardt}, Karl and {Green}, Richard and {Grillmair}, Carl and {Kormendy}, John and {Lauer}, Tod},
        title = "{The Demography of Massive Dark Objects in Galaxy Centers}",
      journal = {\aj},
     keywords = {COSMOLOGY: DARK MATTER, GALAXIES: NUCLEI, Astrophysics},
         year = 1998,
        month = jun,
       volume = {115},
       number = {6},
        pages = {2285-2305},
          doi = {10.1086/300353},
archivePrefix = {arXiv},
       eprint = {astro-ph/9708072},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1998AJ....115.2285M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Koratkar1999,
       author = {{Koratkar}, Anuradha and {Blaes}, Omer},
        title = "{The Ultraviolet and Optical Continuum Emission in Active Galactic Nuclei: The Status of Accretion Disks}",
      journal = {\pasp},
     keywords = {ACCRETION, ACCRETION DISKS, POLARIZATION, GALAXIES: QUASARS: GENERAL, ULTRAVIOLET EMISSION, INVITED REVIEWS},
         year = 1999,
        month = jan,
       volume = {111},
       number = {755},
        pages = {1-30},
          doi = {10.1086/316294},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1999PASP..111....1K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Capellupo2015,
       author = {{Capellupo}, D.~M. and {Netzer}, H. and {Lira}, P. and {Trakhtenbrot}, B. and {Mej{\'\i}a-Restrepo}, Juli{\'a}n},
        title = "{Active galactic nuclei at z {\ensuremath{\sim}} 1.5 - I. Spectral energy distribution and accretion discs}",
      journal = {\mnras},
     keywords = {accretion, accretion discs, galaxies: active, quasars: general, Astrophysics - Astrophysics of Galaxies},
         year = 2015,
        month = feb,
       volume = {446},
       number = {4},
        pages = {3427-3446},
          doi = {10.1093/mnras/stu2266},
archivePrefix = {arXiv},
       eprint = {1410.8137},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015MNRAS.446.3427C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@article{10.1093/mnras/stx718,
    author = {Jin, Chichuan and Done, Chris and Ward, Martin},
    title = "{Super-Eddington QSO RX J0439.6−5311 – I. Origin of the soft X-ray excess and structure of the inner accretion flow}",
    journal = {Monthly Notices of the Royal Astronomical Society},
    volume = {468},
    number = {3},
    pages = {3663-3681},
    year = {2017},
    month = {03},
    abstract = "{We report the results from a recent 133 ks XMM–Newton observation of a highly super-Eddington narrow-line Type-1 quasi-stellar object RX J0439.6−5311. This source has one of the steepest active galactic nuclei hard X-ray slopes, in addition to a prominent and smooth soft X-ray excess. Strong variations are found throughout the 0.3–10 keV energy range on all time-scales covered by the observation, with the soft excess mainly showing low-frequency (LF) variations below 0.1 mHz while the hard X-rays show stronger variability at higher frequencies. We perform a full set of spectral-timing analysis on the X-ray data, including a simultaneous modelling of the time-averaged spectra, frequency-dependent root-mean-square and covariance spectra, lag-frequency and lag-energy spectra. Especially, we find a significant time-lag signal in the LF band, which indicates that the soft X-rays lead the hard by ∼4 ks, with a broad continuum-like profile in the lag spectrum. Our analysis strongly supports the model where the soft X-ray excess is dominated by a separate low temperature, optically thick Comptonization component rather than relativistic reflection or a jet. This soft X-ray emitting region is several tens or hundreds of Rg away from the hot corona emitting hard X-rays, and is probably associated with a geometrically thick (‘puffed-up’) inner disc region.}",
    issn = {0035-8711},
    doi = {10.1093/mnras/stx718},
    url = {https://doi.org/10.1093/mnras/stx718},
    eprint = {https://academic.oup.com/mnras/article-pdf/468/3/3663/13865410/stx718.pdf},
}




@ARTICLE{2016MNRAS.455..691J,
       author = {{Jin}, Chichuan and {Done}, Chris and {Ward}, Martin},
        title = "{Strong constraints on a super-Eddington accretion flow: XMM-Newton observations of an intermediate-mass black hole}",
      journal = {\mnras},
     keywords = {accretion, accretion discs, galaxies: nuclei, galaxies: Seyfert, X-rays: galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2016,
        month = jan,
       volume = {455},
       number = {1},
        pages = {691-702},
          doi = {10.1093/mnras/stv2319},
archivePrefix = {arXiv},
       eprint = {1504.06190},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016MNRAS.455..691J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@INPROCEEDINGS{2018rnls.confE..15K,
       author = {{Komossa}, S.},
        title = "{Multi-wavelength properties of radio-loud Narrow-line Seyfert 1 galaxies}",
     keywords = {Astrophysics - Astrophysics of Galaxies, Astrophysics - High Energy Astrophysical Phenomena},
    booktitle = {Revisiting Narrow-Line Seyfert 1 Galaxies and their Place in the Universe},
         year = 2018,
        month = apr,
          eid = {15},
        pages = {15},
archivePrefix = {arXiv},
       eprint = {1807.03666},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018rnls.confE..15K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Komossa_2006,
	doi = {10.1086/505043},
	url = {https://doi.org/10.1086/505043},
	year = 2006,
	month = {jun},
	publisher = {American Astronomical Society},
	volume = {132},
	number = {2},
	pages = {531--545},
	author = {Stefanie Komossa and Wolfgang Voges and Dawei Xu and Smita Mathur and Hans-Martin Adorf and Gerard Lemson and Wolfgang J. Duschl and Dirk Grupe},
	title = {Radio-loud Narrow-Line Type 1 Quasars},
	journal = {The Astronomical Journal},
	abstract = {We present the first systematic study of (non-radio-selected) radio-loud narrow-line Seyfert 1 (NLS1) galaxies. Cross-correlation of the Catalogue of Quasars and Active Nuclei with several radio and optical catalogs led to the identification of ∼11 radio-loud NLS1 candidates, including four previously known ones. This study almost triples the number of known radio-loud NLS1 galaxies if all candidates are confirmed. Most of the radio-loud NLS1 galaxies are compact, steep-spectrum sources accreting close to or above the Eddington limit. The radio-loud NLS1 galaxies of our sample are remarkable in that they occupy a previously rarely populated regime in NLS1 multiwavelength parameter space. While their [O III]/Hβ and Fe II/Hβ intensity ratios almost cover the whole range observed in NLS1 galaxies, their radio properties extend the range of radio-loud objects to those with small widths of the broad Balmer lines. Their black hole masses are generally at the upper observed end among NLS1 galaxies but are still unusually small in view of the radio loudness of the sources. Among the radio-detected NLS1 galaxies, the radio index R is distributed quite smoothly up to the critical value of R ≃ 10 and covers about 4 orders of magnitude in total. Statistics show that ∼7% of the NLS1 galaxies are formally radio-loud, while only 2.5% exceed a radio index R > 100. Implications for NLS1 models are discussed. Several mechanisms are considered as explanations for the radio loudness of the NLS1 galaxies and for the lower frequency of radio-loud galaxies among NLS1 galaxies than among quasars. While properties of most sources (with two to three exceptions) generally do not favor relativistic beaming, the combination of accretion mode and spin may explain the observations.}
}
@ARTICLE{2009PASJ...61..769K,
       author = {{Kawashima}, Tomohisa and {Ohsuga}, Ken and {Mineshige}, Shin and {Heinzeller}, Dominikus and {Takabe}, Hideaki and {Matsumoto}, Ryoji},
        title = "{New Spectral State of Supercritical Accretion Flow with Comptonizing Outflow}",
      journal = {\pasj},
     keywords = {accretion, accretion disks, black hole physics, hydrodynamics, radiative transfer, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2009,
        month = aug,
       volume = {61},
        pages = {769},
          doi = {10.1093/pasj/61.4.769},
archivePrefix = {arXiv},
       eprint = {0904.4123},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009PASJ...61..769K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Wang2014a,
       author = {{Wang}, Jian-Min and {Du}, Pu and {Hu}, Chen and {Netzer}, Hagai and {Bai}, Jin-Ming and {Lu}, Kai-Xing and {Kaspi}, Shai and {Qiu}, Jie and {Li}, Yan-Rong and {Wang}, Fang and {SEAMBH Collaboration}},
        title = "{Supermassive Black Holes with High Accretion Rates in Active Galactic Nuclei. II. The Most Luminous Standard Candles in the Universe}",
      journal = {\apj},
     keywords = {accretion, accretion disks, cosmology: observations, galaxies: active, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2014,
        month = oct,
       volume = {793},
       number = {2},
          eid = {108},
        pages = {108},
          doi = {10.1088/0004-637X/793/2/108},
archivePrefix = {arXiv},
       eprint = {1408.2337},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...793..108W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Wang2003,
       author = {{Wang}, J. -M. and {Netzer}, H.},
        title = "{Extreme slim accretion disks and narrow line Seyfert 1 galaxies: The nature of the soft X-ray hump}",
      journal = {\aap},
     keywords = {accretion, accretion disks, galaxies: active, galaxies: Seyfert, X-rays: galaxies, Astrophysics},
         year = 2003,
        month = feb,
       volume = {398},
        pages = {927-936},
          doi = {10.1051/0004-6361:20021511},
archivePrefix = {arXiv},
       eprint = {astro-ph/0210361},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003A&A...398..927W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Porquet2004,
       author = {{Porquet}, D. and {Reeves}, J.~N. and {O'Brien}, P. and {Brinkmann}, W.},
        title = "{XMM-Newton EPIC observations of 21 low-redshift PG quasars}",
      journal = {\aap},
     keywords = {galaxies: quasars: general, X-rays: general, galaxies: nuclei, radiation mechanisms : general, Astrophysics},
         year = 2004,
        month = jul,
       volume = {422},
        pages = {85-95},
          doi = {10.1051/0004-6361:20047108},
archivePrefix = {arXiv},
       eprint = {astro-ph/0404385},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004A&A...422...85P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Piconcelli2005,
       author = {{Piconcelli}, E. and {Jimenez-Bail{\'o}n}, E. and {Guainazzi}, M. and {Schartel}, N. and {Rodr{\'\i}guez-Pascual}, P.~M. and {Santos-Lle{\'o}}, M.},
        title = "{The XMM-Newton view of PG quasars.  I. X-ray continuum and absorption}",
      journal = {\aap},
     keywords = {galaxies: active, galaxies: nuclei, galaxies quasars: general, X-rays: galaxies, Astrophysics},
         year = 2005,
        month = mar,
       volume = {432},
       number = {1},
        pages = {15-30},
          doi = {10.1051/0004-6361:20041621},
archivePrefix = {arXiv},
       eprint = {astro-ph/0411051},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005A&A...432...15P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Du2014,
       author = {{Du}, Pu and {Hu}, Chen and {Lu}, Kai-Xing and {Wang}, Fang and {Qiu}, Jie and {Li}, Yan-Rong and {Bai}, Jin-Ming and {Kaspi}, Shai and {Netzer}, Hagai and {Wang}, Jian-Min and {SEAMBH Collaboration}},
        title = "{Supermassive Black Holes with High Accretion Rates in Active Galactic Nuclei. I. First Results from a New Reverberation Mapping Campaign}",
      journal = {\apj},
     keywords = {accretion, accretion disks, black hole physics, galaxies: active, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2014,
        month = feb,
       volume = {782},
       number = {1},
          eid = {45},
        pages = {45},
          doi = {10.1088/0004-637X/782/1/45},
archivePrefix = {arXiv},
       eprint = {1310.4107},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...782...45D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Du2018,
       author = {{Du}, Pu and {Zhang}, Zhi-Xiang and {Wang}, Kai and {Huang}, Ying-Ke and {Zhang}, Yue and {Lu}, Kai-Xing and {Hu}, Chen and {Li}, Yan-Rong and {Bai}, Jin-Ming and {Bian}, Wei-Hao and {Yuan}, Ye-Fei and {Ho}, Luis C. and {Wang}, Jian-Min and {SEAMBH Collaboration}},
        title = "{Supermassive Black Holes with High Accretion Rates in Active Galactic Nuclei. IX. 10 New Observations of Reverberation Mapping and Shortened H{\ensuremath{\beta}} Lags}",
      journal = {\apj},
     keywords = {accretion, accretion disks, galaxies: active, galaxies: nuclei, quasars: supermassive black holes, Astrophysics - Astrophysics of Galaxies},
         year = 2018,
        month = mar,
       volume = {856},
       number = {1},
          eid = {6},
        pages = {6},
          doi = {10.3847/1538-4357/aaae6b},
archivePrefix = {arXiv},
       eprint = {1802.03022},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJ...856....6D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@article{10.1046/j.1365-8711.1999.02811.x,
    author = {Vaughan, S. and Reeves, J. and Warwick, R. and Edelson, R.},
    title = "{X-ray spectral complexity in narrow-line Seyfert 1 galaxies}",
    journal = {Monthly Notices of the Royal Astronomical Society},
    volume = {309},
    number = {1},
    pages = {113-124},
    year = {1999},
    month = {10},
    issn = {0035-8711},
    doi = {10.1046/j.1365-8711.1999.02811.x},
    url = {https://doi.org/10.1046/j.1365-8711.1999.02811.x},
    eprint = {https://academic.oup.com/mnras/article-pdf/309/1/113/3963390/309-1-113.pdf},
}
@ARTICLE{2012yCat..35420083P,
       author = {{Ponti}, G. and {Papadakis}, I. and {Bianchi}, S. and {Guainazzi}, M. and {Matt}, G. and {Uttley}, P. and {Bonilla}, N.~F.},
        title = "{VizieR Online Data Catalog: CAIXA. II. AGNs from excess variance analysis (Ponti+, 2012)}",
      journal = {VizieR Online Data Catalog},
     keywords = {Active gal. nuclei, X-ray sources},
         year = 2012,
        month = jan,
          eid = {J/A+A/542/A83},
        pages = {J/A+A/542/A83},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012yCat..35420083P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{1980A&A....86..121S,
       author = {{Sunyaev}, R.~A. and {Titarchuk}, L.~G.},
        title = "{Comptonization of X-rays in plasma clouds. Typical radiation spectra.}",
      journal = {\aap},
     keywords = {Compton Effect, Plasma Clouds, Radiative Transfer, X Ray Scattering, X Ray Sources, Electron Plasma, Iron, Line Shape, Plasma Radiation, Plasma Temperature, Astrophysics},
         year = 1980,
        month = jun,
       volume = {500},
        pages = {167-184},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1980A&A....86..121S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1993ApJ...413..507H,
       author = {{Haardt}, Francesco and {Maraschi}, Laura},
        title = "{X-Ray Spectra from Two-Phase Accretion Disks}",
      journal = {\apj},
     keywords = {Accretion Disks, Active Galactic Nuclei, Compton Effect, Electron Energy, Stellar Luminosity, X Ray Spectra, Astronomical Models, Black Body Radiation, Stellar Coronas, X Ray Astronomy, Astrophysics, GALAXIES: ACTIVE, X-RAYS: GALAXIES, ACCRETION, ACCRETION DISKS},
         year = 1993,
        month = aug,
       volume = {413},
        pages = {507},
          doi = {10.1086/173020},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1993ApJ...413..507H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2001ApJ...547..684M,
       author = {{Markowitz}, A. and {Edelson}, R.},
        title = "{An RXTE Survey of Long-Term X-Ray Variability in Seyfert 1 Galaxies}",
      journal = {\apj},
     keywords = {Galaxies: Active, Galaxies: Seyfert, X-Rays: Galaxies, Astrophysics},
         year = 2001,
        month = feb,
       volume = {547},
       number = {2},
        pages = {684-692},
          doi = {10.1086/318402},
archivePrefix = {arXiv},
       eprint = {astro-ph/0009422},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001ApJ...547..684M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1992ApJS...80..109B,
       author = {{Boroson}, Todd A. and {Green}, Richard F.},
        title = "{The Emission-Line Properties of Low-Redshift Quasi-stellar Objects}",
      journal = {\apjs},
     keywords = {Emission Spectra, Line Spectra, Quasars, Seyfert Galaxies, Astronomical Spectroscopy, Computational Astrophysics, Principal Components Analysis, Red Shift, Sky Surveys (Astronomy), Astrophysics, GALAXIES: SEYFERT, GALAXIES: QUASARS: GENERAL, SURVEYS},
         year = 1992,
        month = may,
       volume = {80},
        pages = {109},
          doi = {10.1086/191661},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1992ApJS...80..109B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{1999ApJS..125..297L,
       author = {{Leighly}, Karen M.},
        title = "{A Comprehensive Spectral and Variability Study of Narrow-Line Seyfert 1 Galaxies Observed by ASCA. I. Observations and Time Series Analysis}",
      journal = {\apjs},
     keywords = {GALAXIES: ACTIVE, GALAXIES: SEYFERT, SURVEYS, X-RAYS: GALAXIES, Galaxies: Active, Galaxies: Seyfert, Surveys, X-Rays: Galaxies, Astrophysics},
         year = 1999,
        month = dec,
       volume = {125},
       number = {2},
        pages = {297-316},
          doi = {10.1086/313277},
archivePrefix = {arXiv},
       eprint = {astro-ph/9907294},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1999ApJS..125..297L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{1997MNRAS.285L..25B,
       author = {{Brandt}, W.~N. and {Mathur}, S. and {Elvis}, M.},
        title = "{A comparison of the hard ASCA spectral slopes of broad- and narrow-line Seyfert 1 galaxies}",
      journal = {\mnras},
     keywords = {GALAXIES: ACTIVE, X-RAYS: GALAXIES, Astrophysics},
         year = 1997,
        month = mar,
       volume = {285},
       number = {3},
        pages = {L25-L30},
          doi = {10.1093/mnras/285.3.L25},
archivePrefix = {arXiv},
       eprint = {astro-ph/9703100},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1997MNRAS.285L..25B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1996A&A...309...81W,
       author = {{Wang}, T. and {Brinkmann}, W. and {Bergeron}, J.},
        title = "{X-ray properties of active galactic nuclei with optical FeII emission.}",
      journal = {\aap},
     keywords = {GALAXIES: ACTIVE, X-RAYS: GALAXIES, UV: GALAXIES},
         year = 1996,
        month = may,
       volume = {309},
        pages = {81-96},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1996A&A...309...81W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{1996A&A...305...53B,
       author = {{Boller}, T. and {Brandt}, W.~N. and {Fink}, H.},
        title = "{Soft X-ray properties of narrow-line Seyfert 1 galaxies.}",
      journal = {\aap},
     keywords = {GALAXIES: ACTIVE, GALAXIES: SEYFERT, X-RAYS: GALAXIES, Astrophysics},
         year = 1996,
        month = jan,
       volume = {305},
        pages = {53},
archivePrefix = {arXiv},
       eprint = {astro-ph/9504093},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1996A&A...305...53B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2000A&A...354..411K,
       author = {{Komossa}, Stefanie and {Meerschweinchen}, Janek},
        title = "{X-ray emission/absorption mechanisms of 4 NLSy-1-like AGN and a radio quasar. QSO 0117-2837, RX J0134.3-4258, NGC 4051, Mrk 1298, 4C +74.26}",
      journal = {\aap},
     keywords = {GALAXIES: ACTIVE, GALAXIES: NUCLEI, GALAXIES: QUASARS: GENERAL, GALAXIES: SEYFERT, X-RAYS: GALAXIES, Astrophysics},
         year = 2000,
        month = feb,
       volume = {354},
        pages = {411-422},
archivePrefix = {arXiv},
       eprint = {astro-ph/9911429},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000A&A...354..411K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Boller_2002,
   title={XMM-Newtondiscovery of a sharp spectral feature at ∼ 7 keV in the narrow-line Seyfert 1 galaxy 1H 0707−495},
   volume={329},
   ISSN={1365-2966},
   url={http://dx.doi.org/10.1046/j.1365-8711.2002.05040.x},
   DOI={10.1046/j.1365-8711.2002.05040.x},
   number={1},
   journal={Monthly Notices of the Royal Astronomical Society},
   publisher={Oxford University Press (OUP)},
   author={Boller, TH. and Fabian, A.C. and Sunyaev, R. and Trümper, J. and Vaughan, S. and Ballantyne, D.R. and Brandt, W.N. and Keil, R. and Iwasawa, K.},
   year={2002},
   month={Jan},
   pages={L1–L5}
}
@ARTICLE{2014Natur.513..210S,
       author = {{Shen}, Yue and {Ho}, Luis C.},
        title = "{The diversity of quasars unified by accretion and orientation}",
      journal = {\nat},
     keywords = {Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2014,
        month = sep,
       volume = {513},
       number = {7517},
        pages = {210-213},
          doi = {10.1038/nature13712},
archivePrefix = {arXiv},
       eprint = {1409.2887},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014Natur.513..210S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2008ARA&A..46..475H,
       author = {{Ho}, L.~C.},
        title = "{Nuclear activity in nearby galaxies.}",
      journal = {\araa},
     keywords = {Astrophysics},
         year = 2008,
        month = sep,
       volume = {46},
        pages = {475-539},
          doi = {10.1146/annurev.astro.45.051806.110546},
archivePrefix = {arXiv},
       eprint = {0803.2268},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008ARA&A..46..475H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@INPROCEEDINGS{2018rnls.confE..34G,
       author = {{Gallo}, L.},
        title = "{X-ray perspective of Narrow-line Seyfert 1 galaxies}",
     keywords = {Astrophysics - High Energy Astrophysical Phenomena},
    booktitle = {Revisiting Narrow-Line Seyfert 1 Galaxies and their Place in the Universe},
         year = 2018,
        month = apr,
          eid = {34},
        pages = {34},
archivePrefix = {arXiv},
       eprint = {1807.09838},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018rnls.confE..34G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@article{10.1093/mnras/stu2618,
    author = {Ludlam, R. M. and Cackett, E. M. and Gültekin, K. and Fabian, A. C. and Gallo, L. and Miniutti, G.},
    title = "{X-ray spectral and variability properties of low-mass active galactic nuclei}",
    journal = {Monthly Notices of the Royal Astronomical Society},
    volume = {447},
    number = {3},
    pages = {2112-2122},
    year = {2015},
    month = {01},
    abstract = "{We study the X-ray properties of a sample of 14 optically selected low-mass active galactic nuclei (AGN) whose masses lie within the range 105–2 × 106 M⊙ with XMM–Newton. Only six of these low-mass AGN have previously been studied with sufficient quality X-ray data, thus, we have more than double the number of low-mass AGN observed by XMM–Newton with the addition of our sample. We analyse their X-ray spectral properties and variability and compare the results to their more massive counterparts. The presence of a soft X-ray excess is detectable in all five objects which were not background dominated at 2–3 keV. Combined with previous studies, this gives a total of eight low-mass AGN with a soft excess. The low-mass AGN exhibit rapid, short-term variability (hundreds to thousands of seconds) and long-term variability (months to years). There is a well-known anticorrelation between black hole mass and variability amplitude (normalized excess variance). Comparing our sample of low-mass AGN with this relation we find that all of our sample lie below an extrapolation of the linear relation. Such a flattening of the relation at low masses (below ∼106 M⊙) is expected if the variability in all AGN follows the same shape power spectrum with a break frequency that is dependent on mass. Finally, we also found two objects that show significant absorption in their X-ray spectrum, indicative of type 2 objects, although they are classified as type 1 AGN based on optical spectra.}",
    issn = {0035-8711},
    doi = {10.1093/mnras/stu2618},
    url = {https://doi.org/10.1093/mnras/stu2618},
    eprint = {https://academic.oup.com/mnras/article-pdf/447/3/2112/9387161/stu2618.pdf},
}


@ARTICLE{2007MNRAS.374L..15D,
       author = {{Done}, Chris and {Sobolewska}, Ma{\l}gorzata A. and {Gierli{\'n}ski}, Marek and {Schurch}, Nicholas J.},
        title = "{The iron K feature in narrow line Seyfert 1 galaxies: evidence for a P Cygni profile?}",
      journal = {\mnras},
     keywords = {accretion, accretion discs, atomic processes, line: profiles, galaxies: active, X-rays: galaxies, Astrophysics},
         year = 2007,
        month = jan,
       volume = {374},
       number = {1},
        pages = {L15-L19},
          doi = {10.1111/j.1745-3933.2006.00255.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0610078},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007MNRAS.374L..15D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2009Natur.459..540F,
       author = {{Fabian}, A.~C. and {Zoghbi}, A. and {Ross}, R.~R. and {Uttley}, P. and {Gallo}, L.~C. and {Brandt}, W.~N. and {Blustin}, A.~J. and {Boller}, T. and {Caballero-Garcia}, M.~D. and {Larsson}, J. and {Miller}, J.~M. and {Miniutti}, G. and {Ponti}, G. and {Reis}, R.~C. and {Reynolds}, C.~S. and {Tanaka}, Y. and {Young}, A.~J.},
        title = "{Broad line emission from iron K- and L-shell transitions in the active galaxy 1H0707-495}",
      journal = {\nat},
         year = 2009,
        month = may,
       volume = {459},
       number = {7246},
        pages = {540-542},
          doi = {10.1038/nature08007},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009Natur.459..540F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2013MNRAS.435.1840R,
       author = {{Ricci}, C. and {Paltani}, S. and {Ueda}, Y. and {Awaki}, H.},
        title = "{On the role of the {\ensuremath{\Gamma}} - {\ensuremath{\lambda}}$_{Edd}$ relation on the X-ray Baldwin effect in active galactic nuclei}",
      journal = {\mnras},
     keywords = {galaxies: active, galaxies: nuclei, quasars: emission lines, quasars: general, galaxies: Seyfert, X-rays: galaxies, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2013,
        month = nov,
       volume = {435},
       number = {3},
        pages = {1840-1851},
          doi = {10.1093/mnras/stt1326},
archivePrefix = {arXiv},
       eprint = {1307.4507},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013MNRAS.435.1840R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2014ApJ...795..147R,
       author = {{Ricci}, C. and {Tazaki}, F. and {Ueda}, Y. and {Paltani}, S. and {Boissay}, R. and {Terashima}, Y.},
        title = "{Suzaku Observation of IRAS 00521-7054, a Peculiar Type-II AGN with a Very Broad Feature at 6 keV}",
      journal = {\apj},
     keywords = {accretion, accretion disks, galaxies: nuclei, galaxies: Seyfert, quasars: emission lines, X-rays: galaxies, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2014,
        month = nov,
       volume = {795},
       number = {2},
          eid = {147},
        pages = {147},
          doi = {10.1088/0004-637X/795/2/147},
archivePrefix = {arXiv},
       eprint = {1408.6095},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...795..147R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Walton2020,
       author = {{Walton}, D.~J. and {Alston}, W.~N. and {Kosec}, P. and {Fabian}, A.~C. and {Gallo}, L.~C. and {Garcia}, J.~A. and {Miller}, J.~M. and {Nardini}, E. and {Reynolds}, M.~T. and {Ricci}, C. and {Stern}, D. and {Dauser}, T. and {Harrison}, F.~A. and {Reynolds}, C.~S.},
        title = "{A full characterization of the supermassive black hole in IRAS-=09149-6206}",
      journal = {\mnras},
     keywords = {black hole physics, galaxies: active, X-rays: individual (IRAS-=09149-6206), Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Astrophysics of Galaxies},
         year = 2020,
        month = nov,
       volume = {499},
       number = {1},
        pages = {1480-1498},
          doi = {10.1093/mnras/staa2961},
archivePrefix = {arXiv},
       eprint = {2009.10734},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020MNRAS.499.1480W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@article{Fabian_2002,
   title={How the X-ray spectrum of a narrow-line Seyfert 1 galaxy may be reflection-dominated},
   volume={331},
   ISSN={1365-2966},
   url={http://dx.doi.org/10.1046/j.1365-8711.2002.05419.x},
   DOI={10.1046/j.1365-8711.2002.05419.x},
   number={3},
   journal={Monthly Notices of the Royal Astronomical Society},
   publisher={Oxford University Press (OUP)},
   author={Fabian, A. C. and Ballantyne, D. R. and Merloni, A. and Vaughan, S. and Iwasawa, K. and Boller, Th.},
   year={2002},
   month={Apr},
   pages={L35–L39}
}

@article{Fabian_2004,
   title={X-ray reflection in the narrow-line Seyfert 1 galaxy 1H 0707-495},
   volume={353},
   ISSN={1365-2966},
   url={http://dx.doi.org/10.1111/j.1365-2966.2004.08036.x},
   DOI={10.1111/j.1365-2966.2004.08036.x},
   number={4},
   journal={Monthly Notices of the Royal Astronomical Society},
   publisher={Oxford University Press (OUP)},
   author={Fabian, A. C. and Miniutti, G. and Gallo, L. and Boller, Th. and Tanaka, Y. and Vaughan, S. and Ross, R. R.},
   year={2004},
   month={Oct},
   pages={1071–1077}
}

@ARTICLE{2004MNRAS.349.1435M,
       author = {{Miniutti}, G. and {Fabian}, A.~C.},
        title = "{A light bending model for the X-ray temporal and spectral properties of accreting black holes}",
      journal = {\mnras},
     keywords = {accretion, accretion discs, black hole physics, relativity, galaxies: active, X-rays: galaxies, X-rays: stars, Astrophysics, General Relativity and Quantum Cosmology},
         year = 2004,
        month = apr,
       volume = {349},
       number = {4},
        pages = {1435-1448},
          doi = {10.1111/j.1365-2966.2004.07611.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0309064},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004MNRAS.349.1435M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2006MNRAS.365.1067C,
       author = {{Crummy}, J. and {Fabian}, A.~C. and {Gallo}, L. and {Ross}, R.~R.},
        title = "{An explanation for the soft X-ray excess in active galactic nuclei}",
      journal = {\mnras},
     keywords = {accretion, accretion discs, galaxies: active, X-rays: galaxies, Astrophysics},
         year = 2006,
        month = feb,
       volume = {365},
       number = {4},
        pages = {1067-1081},
          doi = {10.1111/j.1365-2966.2005.09844.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0511457},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006MNRAS.365.1067C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1998MNRAS.301..179M,
       author = {{Magdziarz}, Pawel and {Blaes}, Omer M. and {Zdziarski}, Andrzej A. and {Johnson}, W. Neil and {Smith}, David A.},
        title = "{A spectral decomposition of the variable optical, ultraviolet and X-ray continuum of NGC 5548}",
      journal = {\mnras},
     keywords = {ACCRETION, ACCRETION DISCS, GALAXIES: INDIVIDUAL: NGC 5548, GALAXIES: SEYFERT, ULTRAVIOLET: GALAXIES, X-RAYS: GALAXIES},
         year = 1998,
        month = nov,
       volume = {301},
       number = {1},
        pages = {179-192},
          doi = {10.1046/j.1365-8711.1998.02015.x},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1998MNRAS.301..179M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012MNRAS.420.1848D,
       author = {{Done}, Chris and {Davis}, S.~W. and {Jin}, C. and {Blaes}, O. and {Ward}, M.},
        title = "{Intrinsic disc emission and the soft X-ray excess in active galactic nuclei}",
      journal = {\mnras},
     keywords = {accretion, accretion discs, black hole physics, galaxies: active, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2012,
        month = mar,
       volume = {420},
       number = {3},
        pages = {1848-1860},
          doi = {10.1111/j.1365-2966.2011.19779.x},
archivePrefix = {arXiv},
       eprint = {1107.5429},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012MNRAS.420.1848D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2018A&A...611A..59P,
       author = {{Petrucci}, P. -O. and {Ursini}, F. and {De Rosa}, A. and {Bianchi}, S. and {Cappi}, M. and {Matt}, G. and {Dadina}, M. and {Malzac}, J.},
        title = "{Testing warm Comptonization models for the origin of the soft X-ray excess in AGNs}",
      journal = {\aap},
     keywords = {galaxies: active, galaxies: Seyfert, X-rays: galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2018,
        month = mar,
       volume = {611},
          eid = {A59},
        pages = {A59},
          doi = {10.1051/0004-6361/201731580},
archivePrefix = {arXiv},
       eprint = {1710.04940},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018A&A...611A..59P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2020A&A...634A..85P,
       author = {{Petrucci}, P. -O. and {Gronkiewicz}, D. and {Rozanska}, A. and {Belmont}, R. and {Bianchi}, S. and {Czerny}, B. and {Matt}, G. and {Malzac}, J. and {Middei}, R. and {De Rosa}, A. and {Ursini}, F. and {Cappi}, M.},
        title = "{Radiation spectra of warm and optically thick coronae in AGNs}",
      journal = {\aap},
     keywords = {galaxies: active, radiative transfer, methods: numerical, X-rays: galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2020,
        month = feb,
       volume = {634},
          eid = {A85},
        pages = {A85},
          doi = {10.1051/0004-6361/201937011},
archivePrefix = {arXiv},
       eprint = {2001.02026},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020A&A...634A..85P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2014ApJ...794..111B,
       author = {{Balokovi{\'c}}, M. and {Comastri}, A. and {Harrison}, F.~A. and {Alexander}, D.~M. and {Ballantyne}, D.~R. and {Bauer}, F.~E. and {Boggs}, S.~E. and {Brandt}, W.~N. and {Brightman}, M. and {Christensen}, F.~E. and {Craig}, W.~W. and {Del Moro}, A. and {Gandhi}, P. and {Hailey}, C.~J. and {Koss}, M. and {Lansbury}, G.~B. and {Luo}, B. and {Madejski}, G.~M. and {Marinucci}, A. and {Matt}, G. and {Markwardt}, C.~B. and {Puccetti}, S. and {Reynolds}, C.~S. and {Risaliti}, G. and {Rivers}, E. and {Stern}, D. and {Walton}, D.~J. and {Zhang}, W.~W.},
        title = "{The NuSTAR View of Nearby Compton-thick Active Galactic Nuclei: The Cases of NGC 424, NGC 1320, and IC 2560}",
      journal = {\apj},
     keywords = {galaxies: individual: NGC 424 NGC 1320 IC 2560, galaxies: nuclei, galaxies: Seyfert, techniques: spectroscopic, X-rays: galaxies, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Astrophysics of Galaxies},
         year = 2014,
        month = oct,
       volume = {794},
       number = {2},
          eid = {111},
        pages = {111},
          doi = {10.1088/0004-637X/794/2/111},
archivePrefix = {arXiv},
       eprint = {1408.5414},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...794..111B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2014ApJ...788...61B,
       author = {{Brenneman}, L.~W. and {Madejski}, G. and {Fuerst}, F. and {Matt}, G. and {Elvis}, M. and {Harrison}, F.~A. and {Ballantyne}, D.~R. and {Boggs}, S.~E. and {Christensen}, F.~E. and {Craig}, W.~W. and {Fabian}, A.~C. and {Grefenstette}, B.~W. and {Hailey}, C.~J. and {Madsen}, K.~K. and {Marinucci}, A. and {Rivers}, E. and {Stern}, D. and {Walton}, D.~J. and {Zhang}, W.~W.},
        title = "{The Broad-band X-Ray Spectrum of IC 4329A from a Joint NuSTAR/Suzaku Observation}",
      journal = {\apj},
     keywords = {accretion, accretion disks, galaxies: active, galaxies: individual: IC 4329A, galaxies: nuclei, galaxies: Seyfert, X-rays: galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2014,
        month = jun,
       volume = {788},
       number = {1},
          eid = {61},
        pages = {61},
          doi = {10.1088/0004-637X/788/1/61},
archivePrefix = {arXiv},
       eprint = {1404.7486},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...788...61B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{Tortosa_2016,
   title={Broadband X-ray spectral analysis of the Seyfert 1 galaxy GRS 1734-292},
   ISSN={1365-2966},
   url={http://dx.doi.org/10.1093/mnras/stw3301},
   DOI={10.1093/mnras/stw3301},
   journal={Monthly Notices of the Royal Astronomical Society},
   publisher={Oxford University Press (OUP)},
   author={Tortosa, A. and Marinucci, A. and Matt, G. and Bianchi, S. and Franca, F. La and Ballantyne, D. R. and Boorman, P. G. and Fabian, A.C. and Farrah, D. and Fuerst, F. and et al.},
   year={2016},
   month={Dec},
   pages={stw3301}
}
@ARTICLE{Parker2014,
       author = {{Parker}, M.~L. and {Wilkins}, D.~R. and {Fabian}, A.~C. and {Grupe}, D. and {Dauser}, T. and {Matt}, G. and {Harrison}, F.~A. and {Brenneman}, L. and {Boggs}, S.~E. and {Christensen}, F.~E. and {Craig}, W.~W. and {Gallo}, L.~C. and {Hailey}, C.~J. and {Kara}, E. and {Komossa}, S. and {Marinucci}, A. and {Miller}, J.~M. and {Risaliti}, G. and {Stern}, D. and {Walton}, D.~J. and {Zhang}, W.~W.},
        title = "{The NuSTAR spectrum of Mrk 335: extreme relativistic effects within two gravitational radii of the event horizon?}",
      journal = {\mnras},
     keywords = {galaxies: active, galaxies: individual: Mrk 335, galaxies: Seyfert, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2014,
        month = sep,
       volume = {443},
       number = {2},
        pages = {1723-1732},
          doi = {10.1093/mnras/stu1246},
archivePrefix = {arXiv},
       eprint = {1407.8223},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014MNRAS.443.1723P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@article{Kara_2017,
   title={The high-Eddington NLS1 Ark 564 has the coolest corona},
   volume={468},
   ISSN={1365-2966},
   url={http://dx.doi.org/10.1093/mnras/stx792},
   DOI={10.1093/mnras/stx792},
   number={3},
   journal={Monthly Notices of the Royal Astronomical Society},
   publisher={Oxford University Press (OUP)},
   author={Kara, E. and García, J. A. and Lohfink, A. and Fabian, A. C. and Reynolds, C. S. and Tombesi, F. and Wilkins, D. R.},
   year={2017},
   month={Mar},
   pages={3489–3498}
}
@ARTICLE{2018A&A...614A..37T,
       author = {{Tortosa}, A. and {Bianchi}, S. and {Marinucci}, A. and {Matt}, G. and {Petrucci}, P.~O.},
        title = "{A NuSTAR census of coronal parameters in Seyfert galaxies}",
      journal = {\aap},
     keywords = {galaxies: active, galaxies: Seyfert, X-rays: galaxies, black hole physics, Astrophysics - Astrophysics of Galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2018,
        month = jun,
       volume = {614},
          eid = {A37},
        pages = {A37},
          doi = {10.1051/0004-6361/201732382},
archivePrefix = {arXiv},
       eprint = {1801.04456},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018A&A...614A..37T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Veron2001,
       author = {{V{\'e}ron-Cetty}, M. -P. and {V{\'e}ron}, P. and {Gon{\c{c}}alves}, A.~C.},
        title = "{A spectrophotometric atlas of Narrow-Line Seyfert 1 galaxies}",
      journal = {\aap},
     keywords = {GALAXIES: SEYFERT, Astrophysics},
         year = 2001,
        month = jun,
       volume = {372},
        pages = {730-754},
          doi = {10.1051/0004-6361:20010489},
archivePrefix = {arXiv},
       eprint = {astro-ph/0104151},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001A&A...372..730V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Boller1992,
       author = {{Boller}, Th. and {Meurs}, E.~J.~A. and {Brinkmann}, W. and {Fink}, H. and {Zimmermann}, U. and {Adorf}, H. -M.},
        title = "{ROSAT all sky survey observations of IRAS galaxies.}",
      journal = {\aap},
     keywords = {Elliptical Galaxies, Infrared Sources (Astronomy), Quasars, Rosat Mission, Sky Surveys (Astronomy), X Ray Sources, Astronomical Spectroscopy, Color-Color Diagram, Infrared Astronomy Satellite, Spectral Energy Distribution, Astrophysics},
         year = 1992,
        month = jul,
       volume = {261},
        pages = {57-77},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1992A&A...261...57B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Moran1996,
       author = {{Moran}, Edward C. and {Halpern}, Jules P. and {Helfand}, David J.},
        title = "{Classification of IRAS-selected X-Ray Galaxies in the ROSAT All-Sky Survey}",
      journal = {\apjs},
     keywords = {GALAXIES: SEYFERT, GALAXIES: ACTIVE, INFRARED: GALAXIES, X-RAYS: GALAXIES},
         year = 1996,
        month = oct,
       volume = {106},
        pages = {341},
          doi = {10.1086/192341},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1996ApJS..106..341M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015ApJ...806...22D,
       author = {{Du}, Pu and {Hu}, Chen and {Lu}, Kai-Xing and {Huang}, Ying-Ke and {Cheng}, Cheng and {Qiu}, Jie and {Li}, Yan-Rong and {Zhang}, Yang-Wei and {Fan}, Xu-Liang and {Bai}, Jin-Ming and {Bian}, Wei-Hao and {Yuan}, Ye-Fei and {Kaspi}, Shai and {Ho}, Luis C. and {Netzer}, Hagai and {Wang}, Jian-Min and {SEAMBH Collaboration}},
        title = "{Supermassive Black Holes with High Accretion Rates in Active Galactic Nuclei. IV. H{\ensuremath{\beta}} Time Lags and Implications for Super-Eddington Accretion}",
      journal = {\apj},
     keywords = {accretion, accretion disks, black hole physics, galaxies: active, quasars: supermassive black holes, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2015,
        month = jun,
       volume = {806},
       number = {1},
          eid = {22},
        pages = {22},
          doi = {10.1088/0004-637X/806/1/22},
archivePrefix = {arXiv},
       eprint = {1504.01844},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJ...806...22D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2016MNRAS.459.3738I,
       author = {{Inayoshi}, Kohei and {Haiman}, Zolt{\'a}n and {Ostriker}, Jeremiah P.},
        title = "{Hyper-Eddington accretion flows on to massive black holes}",
      journal = {\mnras},
     keywords = {black hole physics, cosmology: theory, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2016,
        month = jul,
       volume = {459},
       number = {4},
        pages = {3738-3755},
          doi = {10.1093/mnras/stw836},
archivePrefix = {arXiv},
       eprint = {1511.02116},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016MNRAS.459.3738I},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@misc{middleton2021nustar,
      title={NuSTAR reveals the hidden nature of SS433}, 
      author={M. J. Middleton and D. J. Walton and W. Alston and T. Dauser and S. Eikenberry and Y-F Jiang and A. C. Fabian and F. Fuerst and M. Brightman and H. Marshall and M. Parker and C. Pinto and F. A. Harrison and M. Bachetti and D. Altamirano and A. J. Bird and G. Perez and J. Miller-Jones and P. A. Charles and S. Boggs and F. Christensen and W. Craig and K. Forster and B. Grefenstette and C. Hailey and K. Madsen and D. Stern and W. Zhang},
      year={2021},
      eprint={1810.10518},
      archivePrefix={arXiv},
      primaryClass={astro-ph.HE}
}
@ARTICLE{2017AN....338..234P,
       author = {{Pinto}, C. and {Fabian}, A. and {Middleton}, M. and {Walton}, D.},
        title = "{Ultrafast outflows in ultraluminous X-ray sources}",
      journal = {Astronomische Nachrichten},
     keywords = {X-ray binaries: accretion, accretion disks, winds-black hole physics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2017,
        month = mar,
       volume = {338},
       number = {234},
        pages = {234-240},
          doi = {10.1002/asna.201713336},
archivePrefix = {arXiv},
       eprint = {1611.00623},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017AN....338..234P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2020MNRAS.494.6012W,
       author = {{Walton}, D.~J. and {Pinto}, C. and {Nowak}, M. and {Bachetti}, M. and {Sathyaprakash}, R. and {Kara}, E. and {Roberts}, T.~P. and {Soria}, R. and {Brightman}, M. and {Canizares}, C.~R. and {Earnshaw}, H.~P. and {F{\"u}rst}, F. and {Heida}, M. and {Middleton}, M.~J. and {Stern}, D. and {Tao}, L. and {Webb}, N. and {Alston}, W.~N. and {Barret}, D. and {Fabian}, A.~C. and {Harrison}, F.~A. and {Kosec}, P.},
        title = "{The unusual broad-band X-ray spectral variability of NGC 1313 X-1 seen with XMM-Newton, Chandra, and NuSTAR}",
      journal = {\mnras},
     keywords = {X-rays: binaries, X-rays: individual: NGC 1313 X-1, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Astrophysics of Galaxies},
         year = 2020,
        month = jun,
       volume = {494},
       number = {4},
        pages = {6012-6029},
          doi = {10.1093/mnras/staa1129},
archivePrefix = {arXiv},
       eprint = {1911.09622},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020MNRAS.494.6012W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2016MNRAS.461.4496S,
       author = {{Sakurai}, Yuya and {Inayoshi}, Kohei and {Haiman}, Zolt{\'a}n},
        title = "{Hyper-Eddington mass accretion on to a black hole with super-Eddington luminosity}",
      journal = {\mnras},
     keywords = {black hole physics, quasars: supermassive black holes, cosmology: theory, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2016,
        month = oct,
       volume = {461},
       number = {4},
        pages = {4496-4504},
          doi = {10.1093/mnras/stw1652},
archivePrefix = {arXiv},
       eprint = {1605.09105},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016MNRAS.461.4496S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2020ApJ...896....1C,
       author = {{Cackett}, Edward M. and {Gelbord}, Jonathan and {Li}, Yan-Rong and {Horne}, Keith and {Wang}, Jian-Min and {Barth}, Aaron J. and {Bai}, Jin-Ming and {Bian}, Wei-Hao and {Carroll}, Russell W. and {Du}, Pu and {Edelson}, Rick and {Goad}, Michael R. and {Ho}, Luis C. and {Hu}, Chen and {Khatu}, Viraja C. and {Luo}, Bin and {Miller}, Jake and {Yuan}, Ye-Fei},
        title = "{Supermassive Black Holes with High Accretion Rates in Active Galactic Nuclei. XI. Accretion Disk Reverberation Mapping of Mrk 142}",
      journal = {\apj},
     keywords = {Active galactic nuclei, Accretion, 16, 14, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Astrophysics of Galaxies},
         year = 2020,
        month = jun,
       volume = {896},
       number = {1},
          eid = {1},
        pages = {1},
          doi = {10.3847/1538-4357/ab91b5},
archivePrefix = {arXiv},
       eprint = {2005.03685},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJ...896....1C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Walton2021,
       author = {{Walton}, D.~J. and {Heida}, M. and {Bachetti}, M. and {F{\"u}rst}, F. and {Brightman}, M. and {Earnshaw}, H. and {Evans}, P.~A. and {Fabian}, A.~C. and {Grefenstette}, B.~W. and {Harrison}, F.~A. and {Israel}, G.~L. and {Lansbury}, G.~B. and {Middleton}, M.~J. and {Pike}, S. and {Rana}, V. and {Roberts}, T.~P. and {Rodriguez Castillo}, G.~A. and {Salvaterra}, R. and {Song}, X. and {Stern}, D.},
        title = "{A new transient ultraluminous X-ray source in NGC 7090}",
      journal = {\mnras},
     keywords = {stars: black holes, stars: neutron, X-rays: binaries, X-rays: individual (NGC 7090 ULX3), Astrophysics - High Energy Astrophysical Phenomena},
         year = 2021,
        month = feb,
       volume = {501},
       number = {1},
        pages = {1002-1012},
          doi = {10.1093/mnras/staa3666},
archivePrefix = {arXiv},
       eprint = {2011.08870},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021MNRAS.501.1002W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2016MNRAS.458.1839C,
       author = {{Castell{\'o}-Mor}, N. and {Netzer}, H. and {Kaspi}, S.},
        title = "{Super- and sub-Eddington accreting massive black holes: a comparison of slim and thin accretion discs through study of the spectral energy distribution}",
      journal = {\mnras},
     keywords = {accretion, accretion discs, galaxies: active, galaxies: nuclei, galaxies: Seyfert, Astrophysics - Astrophysics of Galaxies},
         year = 2016,
        month = may,
       volume = {458},
       number = {2},
        pages = {1839-1858},
          doi = {10.1093/mnras/stw445},
archivePrefix = {arXiv},
       eprint = {1601.07177},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016MNRAS.458.1839C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{1994ApJS...92..555F,
       author = {{Fabian}, A.~C.},
        title = "{Hot Plasmas and the Generation of Gamma Rays}",
      journal = {\apjs},
     keywords = {Bremsstrahlung, Gamma Rays, High Temperature Plasmas, Pair Production, Space Plasmas, Thermal Plasmas, Active Galactic Nuclei, Black Holes (Astronomy), Compton Effect, Optical Thickness, Thermalization (Energy Absorption), X Ray Spectra, Space Radiation, GAMMA RAYS: THEORY, PLASMAS},
         year = 1994,
        month = jun,
       volume = {92},
        pages = {555},
          doi = {10.1086/192015},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1994ApJS...92..555F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2020MNRAS.497..302T,
       author = {{Takeo}, Eishun and {Inayoshi}, Kohei and {Mineshige}, Shin},
        title = "{Hyper-Eddington accretion flows on to black holes accompanied by powerful outflows}",
      journal = {\mnras},
     keywords = {accretion, accretion discs, black hole physics, cosmology: theory; quasars: supermassive black holes, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Astrophysics of Galaxies},
         year = 2020,
        month = sep,
       volume = {497},
       number = {1},
        pages = {302-317},
          doi = {10.1093/mnras/staa1906},
archivePrefix = {arXiv},
       eprint = {2002.07187},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020MNRAS.497..302T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2014ApJ...784...77G,
       author = {{Gofford}, J. and {Reeves}, J.~N. and {Braito}, V. and {Nardini}, E. and {Costa}, M.~T. and {Matzeu}, G.~A. and {O'Brien}, P. and {Ward}, M. and {Turner}, T.~J. and {Miller}, L.},
        title = "{Revealing the Location and Structure of the Accretion Disk Wind in PDS 456}",
      journal = {\apj},
     keywords = {black hole physics, quasars: individual: PDS456, X-rays: galaxies, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2014,
        month = mar,
       volume = {784},
       number = {1},
          eid = {77},
        pages = {77},
          doi = {10.1088/0004-637X/784/1/77},
archivePrefix = {arXiv},
       eprint = {1402.3700},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...784...77G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Gofford2015,
       author = {{Gofford}, J. and {Reeves}, J.~N. and {McLaughlin}, D.~E. and {Braito}, V. and {Turner}, T.~J. and {Tombesi}, F. and {Cappi}, M.},
        title = "{The Suzaku view of highly ionized outflows in AGN - II. Location, energetics and scalings with bolometric luminosity}",
      journal = {\mnras},
     keywords = {line: identification, galaxies: active, galaxies: nuclei, X-rays: galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2015,
        month = aug,
       volume = {451},
       number = {4},
        pages = {4169-4182},
          doi = {10.1093/mnras/stv1207},
archivePrefix = {arXiv},
       eprint = {1506.00614},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015MNRAS.451.4169G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@article{Crenshaw2012,
   title={FEEDBACK FROM MASS OUTFLOWS IN NEARBY ACTIVE GALACTIC NUCLEI. I. ULTRAVIOLET AND X-RAY ABSORBERS},
   volume={753},
   ISSN={1538-4357},
   url={http://dx.doi.org/10.1088/0004-637X/753/1/75},
   DOI={10.1088/0004-637x/753/1/75},
   number={1},
   journal={The Astrophysical Journal},
   publisher={American Astronomical Society},
   author={Crenshaw, D. M. and Kraemer, S. B.},
   year={2012},
   month={Jun},
   pages={75}
}

@ARTICLE{Tombesi2010,
       author = {{Tombesi}, F. and {Cappi}, M. and {Reeves}, J.~N. and {Palumbo}, G.~G.~C. and {Yaqoob}, T. and {Braito}, V. and {Dadina}, M.},
        title = "{Evidence for ultra-fast outflows in radio-quiet AGNs. I. Detection and statistical incidence of Fe K-shell absorption lines}",
      journal = {\aap},
     keywords = {black hole physics, X-ray: galaxies, galaxies: Seyfert, line: identification, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2010,
        month = oct,
       volume = {521},
          eid = {A57},
        pages = {A57},
          doi = {10.1051/0004-6361/200913440},
archivePrefix = {arXiv},
       eprint = {1006.2858},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010A&A...521A..57T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Tombesi2013,
       author = {{Tombesi}, F. and {Cappi}, M. and {Reeves}, J.~N. and {Nemmen}, R.~S. and {Braito}, V. and {Gaspari}, M. and {Reynolds}, C.~S.},
        title = "{Unification of X-ray winds in Seyfert galaxies: from ultra-fast outflows to warm absorbers}",
      journal = {\mnras},
     keywords = {accretion, accretion discs, black hole physics, galaxies: active, galaxies: Seyfert, X-rays: galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2013,
        month = apr,
       volume = {430},
       number = {2},
        pages = {1102-1117},
          doi = {10.1093/mnras/sts692},
archivePrefix = {arXiv},
       eprint = {1212.4851},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013MNRAS.430.1102T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Tombesi2014,
       author = {{Tombesi}, F. and {Tazaki}, F. and {Mushotzky}, R.~F. and {Ueda}, Y. and {Cappi}, M. and {Gofford}, J. and {Reeves}, J.~N. and {Guainazzi}, M.},
        title = "{Ultrafast outflows in radio-loud active galactic nuclei}",
      journal = {\mnras},
     keywords = {accretion, accretion discs, black hole physics, line: identification, plasmas, galaxies: active, X-rays: galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2014,
        month = sep,
       volume = {443},
       number = {3},
        pages = {2154-2182},
          doi = {10.1093/mnras/stu1297},
archivePrefix = {arXiv},
       eprint = {1406.7252},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014MNRAS.443.2154T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{tarter1969,
       author = {{Tarter}, C. Bruce and {Tucker}, Wallace H. and {Salpeter}, Edwin E.},
        title = "{The Interaction of X-Ray Sources with Optically Thin Environments}",
      journal = {\apj},
         year = 1969,
        month = jun,
       volume = {156},
        pages = {943},
          doi = {10.1086/150026},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1969ApJ...156..943T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Jiang2019,
       author = {{Jiang}, Yan-Fei and {Stone}, James M. and {Davis}, Shane W.},
        title = "{Super-Eddington Accretion Disks around Supermassive Black Holes}",
      journal = {\apj},
     keywords = {accretion, accretion disks, magnetohydrodynamics: MHD, methods: numerical, quasars: supermassive black holes, radiative transfer, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2019,
        month = aug,
       volume = {880},
       number = {2},
          eid = {67},
        pages = {67},
          doi = {10.3847/1538-4357/ab29ff},
archivePrefix = {arXiv},
       eprint = {1709.02845},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...880...67J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Okuda_2021,
   title={Radiative Shocks around Super-Eddington Accreting Black Holes},
   ISSN={1365-2966},
   url={http://dx.doi.org/10.1093/mnras/stab428},
   DOI={10.1093/mnras/stab428},
   journal={Monthly Notices of the Royal Astronomical Society},
   publisher={Oxford University Press (OUP)},
   author={Okuda, Toru and Singh, Chandra B},
   year={2021},
   month={Feb}
}

@ARTICLE{Fabian2015,
       author = {{Fabian}, A.~C. and {Lohfink}, A. and {Kara}, E. and {Parker}, M.~L. and {Vasudevan}, R. and {Reynolds}, C.~S.},
        title = "{Properties of AGN coronae in the NuSTAR era}",
      journal = {\mnras},
     keywords = {accretion, accretion discs, black hole physics, X-rays: binaries, X-rays: galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2015,
        month = aug,
       volume = {451},
       number = {4},
        pages = {4375-4383},
          doi = {10.1093/mnras/stv1218},
archivePrefix = {arXiv},
       eprint = {1505.07603},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015MNRAS.451.4375F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Tombesi2011,
       author = {{Tombesi}, F. and {Cappi}, M. and {Reeves}, J.~N. and {Palumbo}, G.~G.~C. and {Braito}, V. and {Dadina}, M.},
        title = "{Evidence for Ultra-fast Outflows in Radio-quiet Active Galactic Nuclei. II. Detailed Photoionization Modeling of Fe K-shell Absorption Lines}",
      journal = {\apj},
     keywords = {black hole physics, galaxies: active, galaxies: Seyfert, line: identification, plasmas, X-rays: galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2011,
        month = nov,
       volume = {742},
       number = {1},
          eid = {44},
        pages = {44},
          doi = {10.1088/0004-637X/742/1/44},
archivePrefix = {arXiv},
       eprint = {1109.2882},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011ApJ...742...44T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Gofford2013,
       author = {{Gofford}, Jason and {Reeves}, James N. and {Tombesi}, Francesco and {Braito}, Valentina and {Turner}, T. Jane and {Miller}, Lance and {Cappi}, Massimo},
        title = "{The Suzaku view of highly ionized outflows in AGN - I. Statistical detection and global absorber properties}",
      journal = {\mnras},
     keywords = {line: identification, galaxies: active, galaxies: nuclei, X-rays: galaxies, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2013,
        month = mar,
       volume = {430},
       number = {1},
        pages = {60-80},
          doi = {10.1093/mnras/sts481},
archivePrefix = {arXiv},
       eprint = {1211.5810},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013MNRAS.430...60G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{Fabian2017,
    author = {Fabian, A. C. and Lohfink, A. and Belmont, R. and Malzac, J. and Coppi, P.},
    title = "{Properties of AGN coronae in the NuSTAR era – II. Hybrid plasma}",
    journal = {Monthly Notices of the Royal Astronomical Society},
    volume = {467},
    number = {3},
    pages = {2566-2570},
    year = {2017},
    month = {02},
    abstract = "{The corona, a hot cloud of electrons close to the centre of the accretion disc, produces the hard X-ray power-law continuum commonly seen in luminous active galactic nuclei. The continuum has a high-energy turnover, typically in the range of one to several 100 keV and is suggestive of Comptonization by thermal electrons. We are studying hard X-ray spectra of AGN obtained with NuSTAR after correction for X-ray reflection and under the assumption that coronae are compact, being only a few gravitational radii in size as indicated by reflection and reverberation modelling. Compact coronae raise the possibility that the temperature is limited and indeed controlled by electron–positron pair production, as explored earlier (Paper I). Here, we examine hybrid plasmas in which a mixture of thermal and non-thermal particles is present. Pair production from the non-thermal component reduces the temperature leading to a wider temperature range more consistent with observations.}",
    issn = {0035-8711},
    doi = {10.1093/mnras/stx221},
    url = {https://doi.org/10.1093/mnras/stx221},
    eprint = {https://academic.oup.com/mnras/article-pdf/467/3/2566/10875108/stx221.pdf},
}
@ARTICLE{Svensson1984,
       author = {{Svensson}, R.},
        title = "{Steady mildly relativistic thermal plasmas - Processes and properties}",
      journal = {\mnras},
     keywords = {Cosmic Plasma, Plasma Clouds, Relativistic Plasmas, Thermal Plasmas, Bremsstrahlung, Electron-Positron Pairs, Luminosity, Pair Production, Photons, Steady State, Thermodynamic Equilibrium, Astrophysics},
         year = 1984,
        month = jul,
       volume = {209},
        pages = {175-208},
          doi = {10.1093/mnras/209.2.175},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1984MNRAS.209..175S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Stern1995,
       author = {{Stern}, Boris E. and {Poutanen}, Juri and {Svensson}, Roland and {Sikora}, Marek and {Begelman}, Mitchell C.},
        title = "{On the Geometry of the X-Ray--Emitting Region in Seyfert Galaxies}",
      journal = {\apjl},
     keywords = {ACCRETION, ACCRETION DISKS, GAMMA RAYS: THEORY, RADIATION MECHANISMS: THERMAL, RADIATIVE TRANSFER, GALAXIES: SEYFERT, X-RAYS: GENERAL, Astrophysics},
         year = 1995,
        month = aug,
       volume = {449},
        pages = {L13},
          doi = {10.1086/309617},
archivePrefix = {arXiv},
       eprint = {astro-ph/9506035},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1995ApJ...449L..13S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Uttley2005,
       author = {{Uttley}, Philip and {McHardy}, Ian M.},
        title = "{X-ray variability of NGC 3227 and 5506 and the nature of active galactic nucleus `states'}",
      journal = {\mnras},
     keywords = {methods: statistical, galaxies: active, galaxies: individual: NGC 3227, galaxies: individual: NGC 5506, galaxies: Seyfert, X-rays: galaxies},
         year = 2005,
        month = oct,
       volume = {363},
       number = {2},
        pages = {586-596},
          doi = {10.1111/j.1365-2966.2005.09475.x},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005MNRAS.363..586U},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{McHardy2004,
       author = {{McHardy}, I.~M. and {Papadakis}, I.~E. and {Uttley}, P. and {Page}, M.~J. and {Mason}, K.~O.},
        title = "{Combined long and short time-scale X-ray variability of NGC 4051 with RXTE and XMM-Newton}",
      journal = {\mnras},
     keywords = {black hole physics, galaxies: active, galaxies: individual: NGC 4051, X-rays: binaries, X-rays: galaxies, Astrophysics},
         year = 2004,
        month = mar,
       volume = {348},
       number = {3},
        pages = {783-801},
          doi = {10.1111/j.1365-2966.2004.07376.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0311220},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004MNRAS.348..783M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{McHardy2006,
       author = {{McHardy}, I.~M. and {Koerding}, E. and {Knigge}, C. and {Uttley}, P. and {Fender}, R.~P.},
        title = "{Active galactic nuclei as scaled-up Galactic black holes}",
      journal = {\nat},
     keywords = {Astrophysics},
         year = 2006,
        month = dec,
       volume = {444},
       number = {7120},
        pages = {730-732},
          doi = {10.1038/nature05389},
archivePrefix = {arXiv},
       eprint = {astro-ph/0612273},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006Natur.444..730M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Garcia2013,
   title={X-RAY REFLECTED SPECTRA FROM ACCRETION DISK MODELS. III. A COMPLETE GRID OF IONIZED REFLECTION CALCULATIONS},
   volume={768},
   ISSN={1538-4357},
   url={http://dx.doi.org/10.1088/0004-637X/768/2/146},
   DOI={10.1088/0004-637x/768/2/146},
   number={2},
   journal={The Astrophysical Journal},
   publisher={American Astronomical Society},
   author={García, J. and Dauser, T. and Reynolds, C. S. and Kallman, T. R. and McClintock, J. E. and Wilms, J. and Eikmann, W.},
   year={2013},
   month={Apr},
   pages={146}
}
@ARTICLE{Garcia2016,
       author = {{Garc{\'\i}a}, Javier A. and {Fabian}, Andrew C. and {Kallman}, Timothy R. and {Dauser}, Thomas and {Parker}, Michael L. and {McClintock}, Jeffrey E. and {Steiner}, James F. and {Wilms}, J{\"o}rn},
        title = "{The effects of high density on the X-ray spectrum reflected from accretion discs around black holes}",
      journal = {\mnras},
     keywords = {accretion, accretion discs, atomic processes, line: formation, radiative transfer, relativistic processes, X-rays: general, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2016,
        month = oct,
       volume = {462},
       number = {1},
        pages = {751-760},
          doi = {10.1093/mnras/stw1696},
archivePrefix = {arXiv},
       eprint = {1603.05259},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016MNRAS.462..751G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kallman2001,
       author = {{Kallman}, T. and {Bautista}, M.},
        title = "{Photoionization and High-Density Gas}",
      journal = {\apjs},
     keywords = {Atomic Processes, Radiation Mechanisms: Thermal, Radiative Transfer, Ultraviolet: General, X-Rays: General},
         year = 2001,
        month = mar,
       volume = {133},
       number = {1},
        pages = {221-253},
          doi = {10.1086/319184},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001ApJS..133..221K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Asplund2009,
       author = {{Asplund}, Martin and {Grevesse}, Nicolas and {Sauval}, A. Jacques and {Scott}, Pat},
        title = "{The Chemical Composition of the Sun}",
      journal = {\araa},
     keywords = {Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2009,
        month = sep,
       volume = {47},
       number = {1},
        pages = {481-522},
          doi = {10.1146/annurev.astro.46.060407.145222},
archivePrefix = {arXiv},
       eprint = {0909.0948},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009ARA&A..47..481A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Haardt1991,
       author = {{Haardt}, F. and {Maraschi}, L.},
        title = "{A Two-Phase Model for the X-Ray Emission from Seyfert Galaxies}",
      journal = {\apjl},
     keywords = {Accretion Disks, Astronomical Models, Emission Spectra, Seyfert Galaxies, X Ray Spectra, Computational Astrophysics, Galactic Nuclei, Gravitational Effects, Interstellar Magnetic Fields, Magnetic Field Reconnection, Astrophysics, GALAXIES: NUCLEI, X-RAYS: SPECTRA},
         year = 1991,
        month = oct,
       volume = {380},
        pages = {L51},
          doi = {10.1086/186171},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1991ApJ...380L..51H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Laha2014,
       author = {{Laha}, Sibasish and {Guainazzi}, Matteo and {Dewangan}, Gulab C. and {Chakravorty}, Susmita and {Kembhavi}, Ajit K.},
        title = "{Warm absorbers in X-rays (WAX), a comprehensive high-resolution grating spectral study of a sample of Seyfert galaxies - I. A global view and frequency of occurrence of warm absorbers.}",
      journal = {\mnras},
     keywords = {galaxies: active, quasars: absorption lines, quasars: emission lines, quasars: general, galaxies: Seyfert, X-rays: galaxies, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2014,
        month = jul,
       volume = {441},
       number = {3},
        pages = {2613-2643},
          doi = {10.1093/mnras/stu669},
archivePrefix = {arXiv},
       eprint = {1404.0899},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014MNRAS.441.2613L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Garcia2014,
       author = {{Garc{\'\i}a}, J. and {Dauser}, T. and {Lohfink}, A. and {Kallman}, T.~R. and {Steiner}, J.~F. and {McClintock}, J.~E. and {Brenneman}, L. and {Wilms}, J. and {Eikmann}, W. and {Reynolds}, C.~S. and {Tombesi}, F.},
        title = "{Improved Reflection Models of Black Hole Accretion Disks: Treating the Angular Distribution of X-Rays}",
      journal = {\apj},
     keywords = {accretion, accretion disks, black hole physics, galaxies: individual: Ark 120, line: formation, radiative transfer, X-rays: general, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2014,
        month = feb,
       volume = {782},
       number = {2},
          eid = {76},
        pages = {76},
          doi = {10.1088/0004-637X/782/2/76},
archivePrefix = {arXiv},
       eprint = {1312.3231},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...782...76G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Dauser2014,
       author = {{Dauser}, T. and {Garcia}, J. and {Parker}, M.~L. and {Fabian}, A.~C. and {Wilms}, J.},
        title = "{The role of the reflection fraction in constraining black hole spin.}",
      journal = {\mnras},
     keywords = {accretion, accretion discs, black hole physics, line: profiles, galaxies: active, galaxies: nuclei, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2014,
        month = oct,
       volume = {444},
        pages = {L100-L104},
          doi = {10.1093/mnrasl/slu125},
archivePrefix = {arXiv},
       eprint = {1408.2347},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014MNRAS.444L.100D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{8202723,
  author={H. {Yamasaki} and M. {Mizumoto} and K. {Ebisawa} and H. {Sameshima}},
  journal={Publications of the Astronomical Society of Japan}, 
  title={Origin of the characteristic X-ray spectral variations of IRAS 13224−3809}, 
  year={2016},
  volume={68},
  number={5},
  pages={80-80},
  doi={10.1093/pasj/psw070}}


@ARTICLE{1974ApJ...187L...1L,
       author = {{Lightman}, Alan P. and {Eardley}, Douglas M.},
        title = "{Black Holes in Binary Systems: Instability of Disk Accretion}",
      journal = {\apjl},
         year = 1974,
        month = jan,
       volume = {187},
        pages = {L1},
          doi = {10.1086/181377},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1974ApJ...187L...1L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1998ApJ...498L..13K,
       author = {{Krolik}, J.~H.},
        title = "{A New Equilibrium for Accretion Disks Around Black Holes}",
      journal = {\apjl},
     keywords = {ACCRETION, ACCRETION DISKS, GALAXIES: ACTIVE, X-RAYS: GENERAL, Accretion, Accretion Disks, Galaxies: Active, X-Rays: General, Astrophysics},
         year = 1998,
        month = may,
       volume = {498},
       number = {1},
        pages = {L13-L16},
          doi = {10.1086/311298},
archivePrefix = {arXiv},
       eprint = {astro-ph/9802276},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1998ApJ...498L..13K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{2001xeab.confE..71T,
       author = {{Turner}, N.~J. and {Stone}, J.~M. and {Sano}, T.},
        title = "{Accretion and Energy Release in Radiation-Dominated Disks}",
    booktitle = {X-ray Emission from Accretion onto Black Holes},
         year = 2001,
       editor = {{Yaqoob}, T. and {Krolik}, J.~H.},
        month = jan,
          eid = {71},
        pages = {71},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001xeab.confE..71T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{ForemanMackey2013,
	doi = {10.1086/670067},
	url = {https://doi.org/10.1086/670067},
	year = 2013,
	month = {mar},
	publisher = {{IOP} Publishing},
	volume = {125},
	number = {925},
	pages = {306--312},
	author = {Daniel Foreman-Mackey and David W. Hogg and Dustin Lang and Jonathan Goodman},
	title = {emcee: The {MCMC} Hammer},
	journal = {Publications of the Astronomical Society of the Pacific},
	abstract = {We introduce a stable, well tested Python implementation of the affine-invariant ensemble sampler for Markov chain Monte Carlo (MCMC) proposed by Goodman & Weare (2010). The code is open source and has already been used in several published projects in the astrophysics literature. The algorithm behind emcee has several advantages over traditional MCMC sampling methods and it has excellent performance as measured by the autocorrelation time (or function calls per independent sample). One major advantage of the algorithm is that it requires hand-tuning of only 1 or 2 parameters compared to ∼N2 for a traditional algorithm in an N-dimensional parameter space. In this document, we describe the algorithm and the details of our implementation. Exploiting the parallelism of the ensemble method, emcee permits any user to take advantage of multiple CPU cores without extra effort. The code is available online at http://dan.iel.fm/emcee under the GNU General Public License v2.}
}

@article{Foreman-Mackey2016,
  doi = {10.21105/joss.00024},
  url = {https://doi.org/10.21105/joss.00024},
  year = {2016},
  publisher = {The Open Journal},
  volume = {1},
  number = {2},
  pages = {24},
  author = {Daniel Foreman-Mackey},
  title = {corner.py: Scatterplot matrices in Python},
  journal = {Journal of Open Source Software}
}
@ARTICLE{2015ApJS..220....8M,
       author = {{Madsen}, Kristin K. and {Harrison}, Fiona A. and {Markwardt}, Craig B. and {An}, Hongjun and {Grefenstette}, Brian W. and {Bachetti}, Matteo and {Miyasaka}, Hiromasa and {Kitaguchi}, Takao and {Bhalerao}, Varun and {Boggs}, Steve and {Christensen}, Finn E. and {Craig}, William W. and {Forster}, Karl and {Fuerst}, Felix and {Hailey}, Charles J. and {Perri}, Matteo and {Puccetti}, Simonetta and {Rana}, Vikram and {Stern}, Daniel and {Walton}, Dominic J. and {J{\o}rgen Westergaard}, Niels and {Zhang}, William W.},
        title = "{Calibration of the NuSTAR High-energy Focusing X-ray Telescope.}",
      journal = {\apjs},
     keywords = {instrumentation: detectors, space vehicles: instruments, telescopes, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2015,
        month = sep,
       volume = {220},
       number = {1},
          eid = {8},
        pages = {8},
          doi = {10.1088/0067-0049/220/1/8},
archivePrefix = {arXiv},
       eprint = {1504.01672},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJS..220....8M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Petrucci2000,
       author = {{Petrucci}, P.~O. and {Haardt}, F. and {Maraschi}, L. and {Grandi}, P. and {Matt}, G. and {Nicastro}, F. and {Piro}, L. and {Perola}, G.~C. and {De Rosa}, A.},
        title = "{Testing Comptonizing Coronae on a Long BeppoSAX Observation of the Seyfert 1 Galaxy NGC 5548}",
      journal = {\apj},
     keywords = {Galaxies: Active, Galaxies: Individual: NGC Number: NGC 5548, Galaxies: Seyfert, Radiation Mechanisms: Thermal, Astrophysics},
         year = 2000,
        month = sep,
       volume = {540},
       number = {1},
        pages = {131-142},
          doi = {10.1086/309319},
archivePrefix = {arXiv},
       eprint = {astro-ph/0004118},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000ApJ...540..131P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Petrucci2001,
       author = {{Petrucci}, P.~O. and {Haardt}, F. and {Maraschi}, L. and {Grandi}, P. and {Malzac}, J. and {Matt}, G. and {Nicastro}, F. and {Piro}, L. and {Perola}, G.~C. and {De Rosa}, A.},
        title = "{Testing Comptonization Models Using BeppoSAX Observations of Seyfert 1 Galaxies}",
      journal = {\apj},
     keywords = {Galaxies: Active, Galaxies: Seyfert, X-Rays: Galaxies, Astrophysics},
         year = 2001,
        month = aug,
       volume = {556},
       number = {2},
        pages = {716-726},
          doi = {10.1086/321629},
archivePrefix = {arXiv},
       eprint = {astro-ph/0101219},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001ApJ...556..716P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Zdziarski1996,
       author = {{Zdziarski}, A.~A. and {Johnson}, W.~N. and {Magdziarz}, P.},
        title = "{Broad-band {\ensuremath{\gamma}}-ray and X-ray spectra of NGC 4151 and their implications for physical processes and geometry.}",
      journal = {\mnras},
     keywords = {Seyfert Galaxies: X-Ray Spectra, Seyfert Galaxies: Gamma-Ray Spectra, Seyfert Galaxies: Radiation Mechanisms, galaxies: individual: NGC4151 -- galaxies: Seyfert -- gamma-rays: observations -- gamma-rays: theory X-rays: galaxies, Astrophysics},
         year = 1996,
        month = nov,
       volume = {283},
       number = {1},
        pages = {193-206},
          doi = {10.1093/mnras/283.1.193},
archivePrefix = {arXiv},
       eprint = {astro-ph/9607015},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1996MNRAS.283..193Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@article{Zycki1999,
    author = {Życki, Piotr T. and Done, Chris and Smith, David A.},
    title = "{The 1989 May outburst of the soft X-ray transient GS 2023+338 (V404 Cyg)}",
    journal = {Monthly Notices of the Royal Astronomical Society},
    volume = {309},
    number = {3},
    pages = {561-575},
    year = {1999},
    month = {11},
    abstract = "{We reanalyse archival Ginga data of the soft X-ray transient source GS 2023+338 covering the beginning of its 1989 May outburst. The source showed a number of rather unusual features: very high and apparently saturated luminosity, dramatic flux and spectral variability (often on ∼1 s time-scale), and generally very hard spectrum, with no obvious soft thermal component characteristic for soft/high state.We describe the spectrum obtained at the maximum of flux and we demonstrate that it is very different from spectra of other soft X-ray transients at similar luminosity. We confirm previous suggestions that the dramatic variability was the result of heavy and strongly variable photoelectric absorption. We also demonstrate that for a short time the spectrum of the source did look like a typical soft/high state spectrum but that this coincided with very heavy absorption.}",
    issn = {0035-8711},
    doi = {10.1046/j.1365-8711.1999.02885.x},
    url = {https://doi.org/10.1046/j.1365-8711.1999.02885.x},
    eprint = {https://academic.oup.com/mnras/article-pdf/309/3/561/2963416/309-3-561.pdf},
}

@INPROCEEDINGS{Beloborodov1999,
       author = {{Beloborodov}, A.~M.},
        title = "{Accretion Disk Models}",
     keywords = {Astrophysics},
    booktitle = {High Energy Processes in Accreting Black Holes},
         year = 1999,
       editor = {{Poutanen}, Juri and {Svensson}, Roland},
       series = {Astronomical Society of the Pacific Conference Series},
       volume = {161},
        month = jan,
        pages = {295},
archivePrefix = {arXiv},
       eprint = {astro-ph/9901108},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1999ASPC..161..295B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Pozdnyakov1997,
       author = {{Pozdnyakov}, L.~A. and {Sobol}, I.~M. and {Syunyaev}, R.~A.},
        title = "{Effect of the multiple Compton scatterings on an x-ray emission spectrum. Calculation by the Monte Carlo method}",
      journal = {\sovast},
     keywords = {Compton Effect, Cosmic Plasma, Monte Carlo Method, X Ray Sources, X Ray Spectra, Astronomical Models, Emission Spectra, Gamma Rays, X Ray Scattering, Astrophysics},
         year = 1977,
        month = dec,
       volume = {21},
        pages = {708-714},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1977SvA....21..708P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1969ApJ...156..943T,
       author = {{Tarter}, C. Bruce and {Tucker}, Wallace H. and {Salpeter}, Edwin E.},
        title = "{The Interaction of X-Ray Sources with Optically Thin Environments}",
      journal = {\apj},
         year = 1969,
        month = jun,
       volume = {156},
        pages = {943},
          doi = {10.1086/150026},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1969ApJ...156..943T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@misc{kawanaka2021determines,
      title={What Determines Unique Spectra of Super-Eddington Accretors?: Origin of Optically Thick and Low Temperature Coronae in Super-Eddington Accretion Flows}, 
      author={Norita Kawanaka and Shin Mineshige},
      year={2021},
      eprint={2012.05386},
      archivePrefix={arXiv},
      primaryClass={astro-ph.HE}
}
@ARTICLE{2000NewAR..44..503L,
       author = {{Laor}, Ari},
        title = "{Optical, UV, and X-ray clues to the nature of narrow-line AGNs}",
      journal = {\nar},
     keywords = {Astrophysics},
         year = 2000,
        month = sep,
       volume = {44},
       number = {7-9},
        pages = {503-510},
          doi = {10.1016/S1387-6473(00)00088-9},
archivePrefix = {arXiv},
       eprint = {astro-ph/0005144},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000NewAR..44..503L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Pounds1995,
       author = {{Pounds}, K.~A. and {Done}, C. and {Osborne}, J.~P.},
        title = "{RE 1034+39: a high-state Seyfert galaxy?}",
      journal = {\mnras},
     keywords = {ACCRETION, ACCRETION DISCS, GALAXIES: ACTIVE, GALAXIES: INDIVIDUAL: RE 1034+39, GALAXIES: SEYFERT, X-RAYS: GALAXIES},
         year = 1995,
        month = nov,
       volume = {277},
       number = {1},
        pages = {L5-L10},
          doi = {10.1093/mnras/277.1.L5},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1995MNRAS.277L...5P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2009ApJ...699..638H,
       author = {{Ho}, Luis C.},
        title = "{Origin and Dynamical Support of Ionized Gas in Galaxy Bulges}",
      journal = {\apj},
     keywords = {galaxies: active, galaxies: bulges, galaxies: ISM, galaxies: kinematics and dynamics, galaxies: nuclei, galaxies: Seyfert, Astrophysics - Galaxy Astrophysics, Astrophysics - Cosmology and Extragalactic Astrophysics},
         year = 2009,
        month = jul,
       volume = {699},
       number = {1},
        pages = {638-648},
          doi = {10.1088/0004-637X/699/1/638},
archivePrefix = {arXiv},
       eprint = {0906.4103},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009ApJ...699..638H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@misc{koljonen2021almanicer,
      title={ALMA/NICER observations of GRS 1915+105 indicate a return to a hard state}, 
      author={Karri I. I. Koljonen and Talvikki Hovatta},
      year={2021},
      eprint={2102.00693},
      archivePrefix={arXiv},
      primaryClass={astro-ph.HE}
}
@ARTICLE{2005ApJ...627..721G,
       author = {{Greene}, Jenny E. and {Ho}, Luis C.},
        title = "{A Comparison of Stellar and Gaseous Kinematics in the Nuclei of Active Galaxies}",
      journal = {\apj},
     keywords = {Galaxies: Active, Galaxies: Kinematics and Dynamics, Galaxies: Nuclei, Galaxies: Seyfert, Astrophysics},
         year = 2005,
        month = jul,
       volume = {627},
       number = {2},
        pages = {721-732},
          doi = {10.1086/430590},
archivePrefix = {arXiv},
       eprint = {astro-ph/0503675},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005ApJ...627..721G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@article{Krawczyk_2013,
	doi = {10.1088/0067-0049/206/1/4},
	url = {https://doi.org/10.1088/0067-0049/206/1/4},
	year = 2013,
	month = {apr},
	publisher = {American Astronomical Society},
	volume = {206},
	number = {1},
	pages = {4},
	author = {Coleman M. Krawczyk and Gordon T. Richards and Sajjan S. Mehta and Michael S. Vogeley and S. C. Gallagher and Karen M. Leighly and Nicholas P. Ross and Donald P. Schneider},
	title = {{MEAN} {SPECTRAL} {ENERGY} {DISTRIBUTIONS} {AND} {BOLOMETRIC} {CORRECTIONS} {FOR} {LUMINOUS} {QUASARS}},
	journal = {The Astrophysical Journal Supplement Series},
	abstract = {We explore the mid-infrared (mid-IR) through ultraviolet (UV) spectral energy distributions (SEDs) of 119,652 luminous broad-lined quasars with 0.064 < z < 5.46 using mid-IR data from Spitzer and WISE, near-infrared data from the Two Micron All Sky Survey and UKIDSS, optical data from the Sloan Digital Sky Survey, and UV data from the Galaxy Evolution Explorer. The mean SED requires a bolometric correction (relative to 2500 Å) of BC2500 Å =2.75 ± 0.40 using the integrated light from 1 μm–2 keV, and we further explore the range of bolometric corrections exhibited by individual objects. In addition, we investigate the dependence of the mean SED on various parameters, particularly the UV luminosity for quasars with 0.5 ≲ z ≲ 3 and the properties of the UV emission lines for quasars with z ≳ 1.6; the latter is a possible indicator of the strength of the accretion disk wind, which is expected to be SED-dependent. Luminosity-dependent mean SEDs show that, relative to the high-luminosity SED, low-luminosity SEDs exhibit a harder (bluer) far-UV spectral slope (αUV), a redder optical continuum, and less hot dust. Mean SEDs constructed instead as a function of UV emission line properties reveal changes that are consistent with known Principal Component Analysis trends. A potentially important contribution to the bolometric correction is the unseen extreme UV (EUV) continuum. Our work suggests that lower-luminosity quasars and/or quasars with disk-dominated broad emission lines may require an extra continuum component in the EUV that is not present (or much weaker) in high-luminosity quasars with strong accretion disk winds. As such, we consider four possible models and explore the resulting bolometric corrections. Understanding these various SED-dependent effects will be important for accurate determination of quasar accretion rates.}
}
@ARTICLE{2012MNRAS.426..656S,
       author = {{Slone}, Oren and {Netzer}, Hagai},
        title = "{The effects of disc winds on the spectrum and black hole growth rate of active galactic nuclei}",
      journal = {\mnras},
     keywords = {accretion, accretion discs, galaxies: active, galaxies: nuclei, quasars: general, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2012,
        month = oct,
       volume = {426},
       number = {1},
        pages = {656-664},
          doi = {10.1111/j.1365-2966.2012.21699.x},
archivePrefix = {arXiv},
       eprint = {1207.7074},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012MNRAS.426..656S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@article{10.1093/mnras/sty1890,
    author = {Kubota, Aya and Done, Chris},
    title = "{A physical model of the broad-band continuum of AGN and its implications for the UV/X relation and optical variability}",
    journal = {Monthly Notices of the Royal Astronomical Society},
    volume = {480},
    number = {1},
    pages = {1247-1262},
    year = {2018},
    month = {07},
    abstract = "{We develop a new spectral model for the broad-band spectral energy distribution (SED) of active galactic nuclei (AGN). This includes an outer standard disc, an inner warm Comptonizing region to produce the soft X-ray excess and a hot corona. We tie these together energetically by assuming Novikov–Thorne emissivity, and use this to define a size scale for the hard X-ray corona as equal to the radius where the remaining accretion energy down to the black hole can power the observed X-ray emission. We test this on three AGN with well-defined SEDs as well as on larger samples to show that the average hard X-ray luminosity is always approximately a few per cent of the Eddington luminosity across a large range of Eddington ratio. As a consequence, the radial size scale required for gravity to power the X-ray corona has to decrease with increasing Eddington fraction. For the first time, we hardwire this into the spectral models, and set the hard X-ray spectral index self-consistently from the ratio of the hard X-ray luminosity to intercepted seed photon luminosity from the disc. This matches the observed correlation of steeper spectral index with increasing Eddington ratio, as well as reproducing the observed tight UV/X relation of quasars. We also include the reprocessed emission produced by the hot inner flow illuminating the warm Comptonization and standard disc regions and show that this predicts a decreasing amount of optical variability with increasing Eddington ratio as observed, though additional processes may also be required to explain the observed optical variability.}",
    issn = {0035-8711},
    doi = {10.1093/mnras/sty1890},
    url = {https://doi.org/10.1093/mnras/sty1890},
    eprint = {https://academic.oup.com/mnras/article-pdf/480/1/1247/25404545/sty1890.pdf},
}
@ARTICLE{Yoshida2013,
       author = {{Yoshida}, Tessei and {Isobe}, Naoki and {Mineshige}, Shin and {Kubota}, Aya and {Mizuno}, Tsunefumi and {Saitou}, Kei},
        title = "{Two Power-Law States of the Ultraluminous X-Ray Source IC 342 X-1}",
      journal = {\pasj},
     keywords = {accretion, accretion disks, black hole physics, X-rays: individual (IC 342 X-1), Astrophysics - High Energy Astrophysical Phenomena},
         year = 2013,
        month = apr,
       volume = {65},
          eid = {48},
        pages = {48},
          doi = {10.1093/pasj/65.2.48},
archivePrefix = {arXiv},
       eprint = {1212.0994},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013PASJ...65...48Y},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{1988ApJ...332..646A,
       author = {{Abramowicz}, M.~A. and {Czerny}, B. and {Lasota}, J.~P. and {Szuszkiewicz}, E.},
        title = "{Slim Accretion Disks}",
      journal = {\apj},
     keywords = {Accretion Disks, Astronomical Models, Black Holes (Astronomy), Stellar Mass Accretion, Computational Astrophysics, Eddington Approximation, Navier-Stokes Equation, Roche Limit, Astrophysics, BLACK HOLES, STARS: ACCRETION},
         year = 1988,
        month = sep,
       volume = {332},
        pages = {646},
          doi = {10.1086/166683},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1988ApJ...332..646A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Shidatsu2017,
       author = {{Shidatsu}, M. and {Ueda}, Y. and {Fabrika}, S.},
        title = "{NuSTAR and Swift  Observations of the Ultraluminous X-Ray Source IC 342 X-1 in 2016: Witnessing Spectral Evolution}",
      journal = {\apj},
     keywords = {accretion, accretion disks, black hole physics, X-rays: binaries, X-rays: individual: IC 342 X-1, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2017,
        month = apr,
       volume = {839},
       number = {1},
          eid = {46},
        pages = {46},
          doi = {10.3847/1538-4357/aa67e7},
archivePrefix = {arXiv},
       eprint = {1703.06399},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...839...46S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Vierdayanti2010,
       author = {{Vierdayanti}, Kiki and {Mineshige}, Shin and {Ueda}, Yoshihiro},
        title = "{Probing the Peculiar Behavior of GRS 1915+105 at Near-Eddington Luminosity}",
      journal = {\pasj},
     keywords = {accretion, accretion disks, black hole physics, X-rays: individual (GRS 1915+105), Astrophysics - High Energy Astrophysical Phenomena},
         year = 2010,
        month = apr,
       volume = {62},
        pages = {239},
          doi = {10.1093/pasj/62.2.239},
archivePrefix = {arXiv},
       eprint = {1001.3906},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010PASJ...62..239V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1993ApJ...414L..93Z,
       author = {{Zdziarski}, Andrzej A. and {Lightman}, Alan P. and {Maciolek-Niedzwiecki}, Andrzej},
        title = "{Acceleration Efficiency in Nonthermal Sources and the Soft Gamma Rays from NGC 4151 Observed by OSSE and SIGMA}",
      journal = {\apjl},
     keywords = {Astronomical Satellites, Electron Acceleration, Gamma Ray Astronomy, Seyfert Galaxies, Spaceborne Astronomy, Astronomical Models, Electron Energy, Relativistic Electron Beams, Astrophysics, ACCELERATION OF PARTICLES, GALAXIES: INDIVIDUAL NGC NUMBER: NGC 4151, GALAXIES: SEYFERT, RADIATION MECHANISMS: MISCELLANEOUS, X-RAYS: GALAXIES},
         year = 1993,
        month = sep,
       volume = {414},
        pages = {L93},
          doi = {10.1086/187004},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1993ApJ...414L..93Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Serafinelli2019,
       author = {{Serafinelli}, Roberto and {Tombesi}, Francesco and {Vagnetti}, Fausto and {Piconcelli}, Enrico and {Gaspari}, Massimo and {Saturni}, Francesco G.},
        title = "{Multiphase quasar-driven outflows in PG 1114+445. I. Entrained ultra-fast outflows}",
      journal = {\aap},
     keywords = {X-rays: galaxies, quasars: general, quasars: individual: PG 1114+445, galaxies: active, Astrophysics - Astrophysics of Galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2019,
        month = jul,
       volume = {627},
          eid = {A121},
        pages = {A121},
          doi = {10.1051/0004-6361/201935275},
archivePrefix = {arXiv},
       eprint = {1906.02765},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019A&A...627A.121S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Tombesi2012,
       author = {{Tombesi}, F. and {Cappi}, M. and {Reeves}, J.~N. and {Braito}, V.},
        title = "{Evidence for ultrafast outflows in radio-quiet AGNs - III. Location and energetics}",
      journal = {\mnras},
     keywords = {accretion, accretion discs, black hole physics, galaxies: active, X-rays: galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2012,
        month = may,
       volume = {422},
       number = {1},
        pages = {L1-L5},
          doi = {10.1111/j.1745-3933.2012.01221.x},
archivePrefix = {arXiv},
       eprint = {1201.1897},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012MNRAS.422L...1T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Netzer2015,
author = {Netzer, Hagai},
title = {Revisiting the Unified Model of Active Galactic Nuclei},
journal = {Annual Review of Astronomy and Astrophysics},
volume = {53},
number = {1},
pages = {365-408},
year = {2015},
doi = {10.1146/annurev-astro-082214-122302},

URL = { 
        https://doi.org/10.1146/annurev-astro-082214-122302
    
},
eprint = { 
        https://doi.org/10.1146/annurev-astro-082214-122302
    
}
,
    abstract = { This review describes recent developments related to the unified model of active galactic nuclei (AGNs). It focuses on new ideas about the origin and properties of the central obscurer (torus) and the connection to its surroundings. The review does not address radio unification. AGN tori must be clumpy but uncertainties about their properties persist. Today's most promising models involve disk winds of various types and hydrodynamic simulations that link the large-scale galactic disk to the inner accretion flow. Infrared (IR) studies greatly improved our understanding of the spectral energy distribution of AGNs, but they are hindered by various selection effects. X-ray samples are more complete. The dependence of the covering factor of the torus on luminosity is a basic relationship that remains unexplained. There is also much confusion regarding real type-II AGNs, which do not fit into a simple unification scheme. The most impressive recent results are due to IR interferometry, which is not in accord with most torus models, and the accurate mapping of central ionization cones. AGN unification may not apply to merging systems and is possibly restricted to secularly evolving galaxies. }
}
@article{Netzer2013,
    author = {Netzer, Hagai and Trakhtenbrot, Benny},
    title = "{Bolometric luminosity black hole growth time and slim accretion discs in active galactic nuclei}",
    journal = {Monthly Notices of the Royal Astronomical Society},
    volume = {438},
    number = {1},
    pages = {672-679},
    year = {2013},
    month = {12},
    abstract = "{We investigate the accretion rate, bolometric luminosity, black hole (BH) growth time and BH spin in a large active galactic nucleus (AGN) sample under the assumption that all such objects are powered via thin or slim accretion discs (ADs). We use direct estimates of the mass accretion rate, \\$\\dot\\{M\\}\\$, to show that many currently used values of Lbol and L/LEdd are either underestimated or overestimated because they are based on bolometric correction factors that are adjusted to the properties of moderately accreting AGNs and do not take into account the correct combination of BH mass, spin and accretion rate. The consistent application of AD physics to our sample of Sloan Digital Sky Survey (SDSS) AGNs leads to the following findings. (1) Even the most conservative assumption about the radiative efficiency of fast-accreting BHs shows that many of these sources must contain slim ADs. We illustrate this by estimating the fraction of such objects at various redshifts. (2) Many previously estimated BH growth times are inconsistent with the AD theory. In particular, the growth times of the fastest accreting BHs were overestimated in the past by large factors with important consequences to AGN evolution. (3) Currently used bolometric correction factors for low accretion rate very massive SDSS BHs are inconsistent with the AD theory. Applying the AD set of assumptions to such objects, combined with standard photoionization calculations of broad emission lines, leads to the conclusion that many such objects must contain fast-spinning BHs.}",
    issn = {0035-8711},
    doi = {10.1093/mnras/stt2238},
    url = {https://doi.org/10.1093/mnras/stt2238},
    eprint = {https://academic.oup.com/mnras/article-pdf/438/1/672/18466094/stt2238.pdf},
}

@article{Blaes_2001,
	doi = {10.1086/324045},
	url = {https://doi.org/10.1086/324045},
	year = 2001,
	month = {dec},
	publisher = {American Astronomical Society},
	volume = {563},
	number = {2},
	pages = {560--568},
	author = {Omer Blaes and Ivan Hubeny and Eric Agol and Julian H. Krolik},
	title = {Non-{LTE}, Relativistic Accretion Disk Fits to 3C 273 and the Origin of the Lyman Limit Spectral Break},
	journal = {The Astrophysical Journal},
	abstract = {We fit general relativistic, geometrically thin accretion disk models with non-LTE atmospheres to near-simultaneous multiwavelength data of 3C 273, extending from the optical to the far-ultraviolet. Our model fits show no flux discontinuity associated with a hydrogen Lyman edge, but they do exhibit a spectral break which qualitatively resembles that seen in the data. This break arises from relativistic smearing of Lyman emission edges which are produced locally at tens of gravitational radii in the disk. We discuss the possible effects of metal line blanketing on the model spectra, as well as the substantial Comptonization required to explain the observed soft X-ray excess. Our best-fit accretion disk model underpredicts the near-ultraviolet emission in this source and also has an optical spectrum which is too red. We discuss some of the remaining physical uncertainties and suggest in particular that an extension of our models to the slim disk regime and/or including nonzero magnetic torques across the innermost stable circular orbit may help resolve these discrepancies.}
}

@article{Shang_2005,
	doi = {10.1086/426134},
	url = {https://doi.org/10.1086/426134},
	year = 2005,
	month = {jan},
	publisher = {American Astronomical Society},
	volume = {619},
	number = {1},
	pages = {41--59},
	author = {Zhaohui Shang and Michael S. Brotherton and Richard F. Green and Gerard A. Kriss and Jennifer Scott and Jessica Kim Quijano and Omer Blaes and Ivan Hubeny and John Hutchings and Mary Elizabeth Kaiser and Anuradha Koratkar and William Oegerle and Wei Zheng},
	title = {Quasars and the Big Blue Bump},
	journal = {The Astrophysical Journal},
	abstract = {We investigate the ultraviolet-to-optical spectral energy distributions of 17 active galactic nuclei (AGNs) using quasi-simultaneous spectrophotometry spanning 900-9000 Å (rest frame). We employ data from the Far Ultraviolet Spectroscopic Explorer, the Hubble Space Telescope, and the 2.1 m telescope at Kitt Peak National Observatory. Taking advantage of the short-wavelength coverage, we are able to study the so-called big blue bump, the region in which the energy output peaks, in detail. Most objects exhibit a spectral break around 1100 Å. Although this result is formally associated with large uncertainty for some objects, there is strong evidence in the data that the far-ultraviolet spectral region is below the extrapolation of the near-ultraviolet-optical slope, indicating a spectral break around 1100 Å. We compare the behavior of our sample to those of non-LTE thin-disk models covering a range in black hole mass, Eddington ratio, disk inclination, and other parameters. The distribution of ultraviolet-optical spectral indices redward of the break and far-ultraviolet indices shortward of the break are in rough agreement with the models. However, we do not see a correlation between the far-ultraviolet spectral index and the black hole mass, as seen in some accretion disk models. We argue that the observed spectral break is intrinsic to AGNs, although intrinsic reddening as well as Comptonization can strongly affect the far-ultraviolet spectral index. We make our data available online in digital format.}
}
@article{Koratkar_1999,
	doi = {10.1086/316294},
	url = {https://doi.org/10.1086/316294},
	year = 1999,
	month = {jan},
	publisher = {{IOP} Publishing},
	volume = {111},
	number = {755},
	pages = {1--30},
	author = {Anuradha Koratkar and Omer Blaes},
	title = {Invited Review: The Ultraviolet and Optical Continuum Emission in Active Galactic Nuclei: The Status of Accretion Disks},
	journal = {Publications of the Astronomical Society of the Pacific},
	abstract = {A fundamental component of models of active galactic nuclei (AGNs) is an accretion disk around a supermassive black hole. However, the nature of this accretion disk is not well understood, and current models do not provide a satisfactory explanation of the optical/UV continuum observed in AGNs. In this paper we review the substantial theoretical and observational progress made in the field. We also try to point out future research directions that would be fruitful in trying to obtain a complete, self‐consistent model of the continuum‐emitting regions.}
}

@ARTICLE{1999ApJS..125..317L,
       author = {{Leighly}, Karen M.},
        title = "{A Comprehensive Spectral and Variability Study of Narrow-Line Seyfert 1 Galaxies Observed by ASCA. II. Spectral Analysis and Correlations}",
      journal = {\apjs},
     keywords = {GALAXIES: ACTIVE, GALAXIES: SEYFERT, SURVEYS, X-RAYS: GALAXIES, Galaxies: Active, Galaxies: Seyfert, Surveys, X-Rays: Galaxies, Astrophysics},
         year = 1999,
        month = dec,
       volume = {125},
       number = {2},
        pages = {317-348},
          doi = {10.1086/313287},
archivePrefix = {arXiv},
       eprint = {astro-ph/9907295},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1999ApJS..125..317L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2004MNRAS.347..269G,
       author = {{Gallo}, L.~C. and {Boller}, Th. and {Tanaka}, Y. and {Fabian}, A.~C. and {Brandt}, W.~N. and {Welsh}, W.~F. and {Anabuki}, N. and {Haba}, Y.},
        title = "{The X-ray variability of the narrow-line type 1 Seyfert galaxy IRAS 13224-3809 from an XMM-Newton observation}",
      journal = {\mnras},
     keywords = {galaxies: active, galaxies: individual: IRAS 13224, 3809, X-rays: galaxies, Astrophysics},
         year = 2004,
        month = jan,
       volume = {347},
       number = {1},
        pages = {269-276},
          doi = {10.1111/j.1365-2966.2004.07196.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0309169},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004MNRAS.347..269G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2014MNRAS.440.2347M,
       author = {{Marinucci}, A. and {Matt}, G. and {Kara}, E. and {Miniutti}, G. and {Elvis}, M. and {Arevalo}, P. and {Ballantyne}, D.~R. and {Balokovi{\'c}}, M. and {Bauer}, F. and {Brenneman}, L. and {Boggs}, S.~E. and {Cappi}, M. and {Christensen}, F.~E. and {Craig}, W.~W. and {Fabian}, A.~C. and {Fuerst}, F. and {Hailey}, C.~J. and {Harrison}, F.~A. and {Risaliti}, G. and {Reynolds}, C.~S. and {Stern}, D.~K. and {Walton}, D.~J. and {Zhang}, W.},
        title = "{Simultaneous NuSTAR and XMM-Newton 0.5-80 keV spectroscopy of the narrow-line Seyfert 1 galaxy SWIFT J2127.4+5654}",
      journal = {\mnras},
     keywords = {accretion, accretion discs, galaxies: active, galaxies: individual: SWIFT J2127.4+5654, galaxies: Seyfert, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Astrophysics of Galaxies},
         year = 2014,
        month = may,
       volume = {440},
       number = {3},
        pages = {2347-2356},
          doi = {10.1093/mnras/stu404},
archivePrefix = {arXiv},
       eprint = {1402.7245},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014MNRAS.440.2347M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


